Node Connectivity Augmentation via Iterative Randomized Rounding

Many network design problems deal with the design of low-cost networks that are resilient to the failure of their elements, such as nodes or links. One such problem is Connectivity Augmentation, where the goal is to cheaply increase the connectivity of a network from a value k to k+1. The most studied setting focuses on edge-connectivity, which reduces to k=2, called Cactus Augmentation. From an approximation perspective, Byrka, Grandoni, and Jabal Ameli (2020) were the first to break the 2-approximation barrier for this problem, by exploiting a connection to the Steiner Tree problem, and by tailoring the analysis of the iterative randomized rounding technique for Steiner Tree to the specific instances arising from this connection. Recently, Nutov (2020) observed that a similar reduction to Steiner Tree holds for a node-connectivity problem called Block-Tree Augmentation, where the goal is to add edges to a given spanning tree so that the resulting graph 2-node-connected. Combining Nutov's result with the algorithm of Byrka, Grandoni, and Jabal Ameli yields a 1.91-approximation for Block-Tree Augmentation, that is the best bound known so far. In this work, we give a 1.892-approximation algorithm for the problem of augmenting the node-connectivity of any graph from 1 to 2. As a corollary, we improve upon the state-of-the-art approximation factor for Block-Tree Augmentation. Our result is obtained by developing a different and simpler analysis of the iterative randomized rounding technique. Our results also imply a 1.892-approximation algorithm for Cactus Augmentation. While this does not beat the best approximation by Cecchetto, Traub, and Zenklusen (2021) known for this problem, our analysis is quite simple compared to previous results in the literature. In addition, our work gives new insights on the iterative randomized rounding method, that might be of independent interest.

==> appending_binary_trees.tex <==
\subsection{Appending Extended Binary Trees}\label{sec:appending}

We now describe our main procedure that, given a tree $T = (V, E)$ rooted at a vertex $r$, computes a tree spanning the set $F \subseteq V$ of leaves of $T$.

We start by defining the ranking $\pi: F \to [|F|]$ of the leaves that we will use. Algorithm~\ref{alg:generate-ranking} generates a ranking that prioritizes the leaves that are closest to the root, and among them it prioritizes leaves that have more siblings that are leaves.

\begin{algorithm}
Let $Q \leftarrow \arg \min\{|P_T(r,f)|: f \in F\}$.

Let $x \in \arg\max\{|\mathtt{Sibling}_T(f) \cap F|: f \in Q\}$, breaking ties arbitrarily

$\pi(x) \leftarrow 1 + \mathtt{offset}$.

Let $p$ be the closest ancestor of $x$ such that $|\mathtt{Child}_T(p)| > 1$, if any, otherwise let $p \leftarrow \emptyset$.

\eIf{$p \neq \emptyset$}{\Return $\pi \circ \mathtt{GenerateRanking}(T[V \setminus (P_T(p,x) \setminus \{p\}  )], 1 + \mathtt{offset})$}{\Return $\pi$}

\caption{The $\mathtt{GenerateRanking}(T, \mathtt{offset})$ procedure.}
\label{alg:generate-ranking}
\end{algorithm}



The main steps of our procedure are now described in Algorithm~\ref{alg:main-alg}, whose input is a tree $T = (V, E)$ with a set of leaves $F$.

\begin{algorithm}
Pick an arbitrary root $r \in V \setminus F$. From now on, $T$ is assumed to be a tree rooted at $r$.

$\pi \leftarrow \mathtt{GenerateRanking}(T, 0)$.

$(T_0, \mathcal{B}) \leftarrow \mathtt{PartitionIntoBinaryTrees}(T)$

\For{$B \in \{T_0\} \cup \mathcal{B}$}{$G(B) \leftarrow \mathtt{GenerateLeftToRightTree}(B)$}


\Return $\mathtt{AppendTrees}\left(T_0, \mathcal{B}, \{G(B)\}_{B \in \{T_0\} \cup \mathcal{B}} \right)$


\caption{The $\mathtt{GenerateSpanningTree}(T)$ procedure.}
\label{alg:main-alg}
\end{algorithm}

Thus, all that remains to discuss in here is the $\mathtt{AppendTrees}\left(T_0, \mathcal{B}, \{G(B)\}_{B \in \{T_0\} \cup \mathcal{B}} \right)$ procedure, that takes as input a family of extended binary trees along with trees spanning their leaves, and produces a tree spanning all the leaves of the original tree $T$. In order to produce this spanning tree over $F$, we use an iterative procedure that maintains what we call a main tree, which is a subtree of $T$ that increases after each iteration, until it becomes equal to $T$. During each iteration, we consider the main tree and a tree from the family $\mathcal{B}$, and we merge their leaf-spanning trees. We call this procedure ``appending''. Reiterating, we append the trees of $\mathcal{B}$ to the main tree $T'$, which at the beginning is equal to $T_0$, one at a time, until $T' = T$.


\paragraph*{The $\mathtt{AppendTrees}(\ldots)$ procedure} 

The starting point of our analysis are Lemmas~\ref{lemma:extended-binary-tree-properties} and~\ref{lemma:extended-binary-tree-bounds}. In particular, in order to obtain the bound of Lemma~\ref{lemma:extended-binary-tree-bounds}, we assumed that all vertices other than the leafs $\{f_1, \ldots, f_m\}$ and their parents have $w$-value equal to $3$. Thus, whenever the $w$-value of such a vertex is smaller than $3$, then this vertex has some extra budget that it can use in case its $w$-value is increased by the addition of some leaf-to-leaf edge. We now make this more formal. 

Let $B = (V, E)$ be an extended binary tree rooted at a vertex $p$, whose set of leaves is $F$, and let $(f_1, \ldots, f_m)$ be the ordering generated by $\mathtt{GenerateLeftToRightOrdering}(B')$, where $B' = B[(V \setminus F) \cup \mathtt{Marked}(B)]$. For each vertex $u \in V \setminus F$, we define $\mathtt{Budget}_B(u) = \max\{H(3) - H(w(u)), 0\}$. Moreover, for $i \in \{1, m\}$, we define
\begin{equation*}
 \mathtt{Budget}_B(f_i) = 
    \begin{cases} 
      \frac{1}{3}  & \textrm{if }\mathtt{Budget}_B(\mathtt{parent}_B(f_i)) > 0, \\
      \frac{5}{12} & \textrm{if }\mathtt{Budget}_B(\mathtt{parent}_B(f_i)) = 0.
   \end{cases}
\end{equation*}

We will use the budget defined above when appending a tree $B$ to the main tree. We now do some case analysis. From now on, let $T'$ denote the main tree, let $B$ denote the tree we are about to append to the main tree, which is rooted at a vertex $p$ that is connected to a vertex $p' \in T'$ in the original tree $T$. 

We now do some case analysis.


\begin{lemma}
Let $B$ be an extended binary tree rooted at vertex $p$ that is appended to a vertex $p'$ of the main tree $T'$. Then, the new $H$-average will be at most 1.8593.
\end{lemma}
\begin{proof}

    Let $B'$ be the extended binary tree of $T'$ which $p'$ belongs to when we consider the original decomposition $\{T_0\} \cup \mathcal{B}$ of $T$ into extended binary trees. This means that $B'$ is either $T_0$ or an extended binary tree of the set $\mathcal{B}$ that was appended in a prior iteration. Before appending $B$, its leaf-spanning tree $G(B)$ has a $w$ that, by Lemma~\ref{lemma:extended-binary-tree-bounds}, has an $H$-average of at most $1.84$. Let $G(T')$ be the leaf-spanning tree of the main tree. Let $w$ denote the $w$-value of all vertices of $B$ and $T'$ before appending $B$ to $T'$, and $w'$ be the value after appending. In order to connect $G(B)$ with $G(T')$, we will add one edge between $G(B)$ and $G(T')$, based on the ``location'' of $p'$ in $B'$. In all cases, from our decomposition, we must have $|\mathtt{Child}_{B'}(p')| \geq 2$. 
    
    
\begin{itemize}
    \item Case: $\mathtt{Child}_{B'}(p') = \{v_1, v_2, v_3\}$. In this case, $v_1, v_2, v_3$ must all be leaves. So the worst-case increase is incurred when $p'$ is an external node, which is $\frac{1}{4} + \frac{1}{5}$ which can easily be charged to the budget on the exterior path of $B$
    
    \item Case: $|\mathtt{Sibling}(\mathtt{marked}(p))| = 2$. In this case, there two cases for whether $p'$ is part of an external path or not. Suppose $p'$ is part of an external path with $\mathtt{Child}_{B'}(p') = \{v_1, v_2\}$, and w.l.o.g. assume that $v_1$ is on the same external path. In this case, we add the edge $(\mathtt{marked}_{B'}(v_2), \mathtt{marked}_B(p))$. The worst-case increase incurred in the path $P_{B'}(p', \mathtt{marked}_{B'}(v_2))$ is
    \begin{equation*}
        \frac{1}{3} + \frac{|P_{B'}(v_2, \mathtt{marked}_{B'}(v_2))| - 1}{4} + \frac{1}{5}.
    \end{equation*}
    if $p'$ is not part of an external path, then we add the edge $(\mathtt{marked}_{B'}(v_1), \mathtt{marked}_B(p))$ instead. The The worst-case increase incurred in the path $P_{B'}(p', \mathtt{marked}_{B'}(v_1))$ is
    \begin{equation*}
        \frac{|P_{B'}(v_2, \mathtt{marked}_{B'}(v_2))| - 1}{4} + \frac{1}{5} + \frac{1}{6}.
    \end{equation*}
    The amount of budget we have on the external path of $B$ is at least $\frac{|P_{B}(p, \mathtt{marked}_{B} (p))|}{3}$
    
    \item Case: $|\mathtt{Sibling}(\mathtt{marked}(p))| = 3$. In this case, we know by the decomposition that $|\mathtt{Sibling}(\mathtt{marked}(B'_{v_1}))| = |\mathtt{Sibling}(\mathtt{marked}(B'_{v_2}))| = 3$ where $\mathtt{Child}_{B'}(p') = \{v_1, v_2\}$. If $p'$ and $v_1$ are part of the external path of $B'$, then we add the edge $(\mathtt{marked}_{B'}(v_2), \mathtt{marked}_B(p))$, if $p'$ is not part of the external path then we add the edge $(\mathtt{marked}_{B'}(v_1), \mathtt{marked}_B(p))$. The worst case increase incurred in $B'$ is either $\frac{1}{3}$ or $\frac{1}{4}$ depending on if $p'$ is part of the external path of $B'$ or not plus
    \begin{equation*}
        \frac{|P_{B'}(v_2, \mathtt{marked}_{B'}(v_2))| - 2}{4} + \frac{1}{5} + \frac{1}{6}
    \end{equation*}
    
    
    
    
    \item $p'$ is part of an external path of $B'$. We do some further case analysis:
        \begin{itemize}
            \item $\mathtt{Child}_{B'}(p') = \{v_1, v_2\}$ and moreover, $B'_{v_1} \prec B$ and $B'_{v_2} \prec B$. Wlog, assume that $v_1$ is part of the external path of $B'$. In this case, we add the edge $(\mathtt{marked}_{B'}(v_2), \mathtt{marked}_B(p))$. The worst-case increase incurred in the path $P_{B'}(p', \mathtt{marked}_{B'}(v_2))$ is
            \begin{equation*}
                \frac{1}{3} + \frac{|P_{B'}(v_2, \mathtt{marked}_{B'}(v_2))| - 1}{4} + \frac{1}{5}
            \end{equation*}
            Regarding the path $P_{B}(p,\mathtt{marked}_B(p))$, we use the budget of the vertices of the path, and do some case analysis for the last two vertices, $f_1 \coloneqq \mathtt{marked}_B(p))$ and its parent. In the case where $w(\mathtt{parent}_B(f_1))=  2$, the increase on all vertices of the path $P_B(p,\mathtt{parent}_B(f_1))$ can be paid by the budget of each vertex, and so is the increase for the vertex $f_1$, which is either $1/3$ or $1/4$. We will now use the budget of the path 
        \end{itemize}


    \item then if we charge the entire increase to JUST the exterior nodes of $B$ including the 3-stars at its leaves we get the following formula for the new cost of these nodes
        \[
            \frac{1}{2q+3}\left( (q+2)H(2)+(q-2)H(3)+2H(4)+\frac{1}{3} +\frac{q-2}{4}+\frac{1}{5} +\frac{1}{6} \right)
        \]
    \item this formula is maximized for $q=3$ with $1.8592592$
\end{itemize}
\end{proof}


\begin{lemma}
    Let $B$ be an extended binary tree rooted at vertex $p$, with $q=2$, and is appended to a vertex $p'$ of the main tree $T'$. Then, the new $H$-average $T'$ will be at most $1.87921807$.
\end{lemma}
\begin{proof}
    Again, the $H$-average of  $B$ before it is appended to $T'$ is at most $1.84$. 
    
    If $|P_{T'}(p',\mathtt{marked}_{T'}(p'))| = 2$, that is, the level of the node $\mathtt{marked}_{T'}(p')$ is one higher than $\mathtt{marked}_{T'}(p)$ when we attach $B$. Then the worst case is when $p'$ has two children and $B$ has only $3$ nodes. The total cost to the nodes of $B$ in this case is $((H(3)+H(4)+2H(2) + \frac{1}{3}+\frac{1}{4})/4 = 1.875$
    
    Now we consider $|P_{T'}(p',\mathtt{marked}_{T'}(p'))| + 1 = 3$, again the worst case is when $B$ has 3 leaves. Therefore, both the exterior leaves of $T'_{p'}$ have two siblings. 

    the idea here is to charge the increase due to appending $B$ to the nodes on the path it connects to. the worst case here is again when the depth of the parent subtrees are both 3, and thus must have 3-stars at the bottom. therefore, the worst case increase is $1/3 + 1/4 + 1/5 + 1/6$. this cost averaged across the nodes of $B$ will be 
    \[
        \frac{1}{4}\left( 2H(2)+H(3)+H(4)+\frac{1}{3} +\frac{1}{5}+\frac{1}{6} \right) = 1.901417
    \]
    So this is a bad approach, consider instead also charging to the parent of $B$. Since the depth from the parent of $B$ is $3$, the previous lemma applies, so the parent has at most $1.8592592$ charged to it. This means that averaging this way gives
    \[
        \frac{1}{5}\left( 2H(2)+H(3)+H(4)+\frac{1}{3} +\frac{1}{5}+\frac{1}{6} +1.8592592 \right) = 1.895185173...
    \]
    again, not great. so consider charging to the whole path from $p$ to the node we connect to, including the siblings. 
    \[
    \frac{1}{9}\left( 2H(2)+H(3)+H(4)+\frac{1}{3} +\frac{1}{5}+\frac{1}{6} + 5*1.8592592 \right) = 1.87921807
    \]
\end{proof}

The next case does not affect the previous since it requires that the parent has at least 2 leaves in order to be feasible. 
\begin{lemma}
    Let $B$ be an extended binary tree rooted that is just the vertex $\{p\}$, and is appended to a vertex $p'$ of the main tree $T'$. Then, the new $H$-average $T'$ will be at most $1.89337445925$
\end{lemma}
\begin{proof}
    Since $B$ is a single node, we know by our decomposition that $p'$ must already have at least $3$ children. If $u$ is the marked child of $p'$, then we know that the worst-case $w$-values of $p'$ and $u$ are $3$ and $4$ respectively if $p'$ is an external node. By applying the previous lemma and distributing the increase in cost to $B$, $p'$ and $p$, we have that the cost of $T'$ increases to at most 
    \[
    \frac{1}{5}\left( H(2)+\frac{1}{4} +\frac{1}{5} + 4*1.87921807 \right) = 1.89337445925
    \]  

    
\end{proof}

\begin{lemma}
    Let $B$ be an extended binary tree rooted at vertex $p$ that is appended to a vertex $p'$ of the main tree $T'$. Then, the new $H$-average will be at most $1.84365079$ if we allow limited rewiring of the leaf-to-leaf tree of $T'$.
\end{lemma}
\begin{proof}
    This rewiring is done when $B$ is to be appended and the leaf-to-leaf edge $(v,\mathtt{marked}_B(p))$ will be added. So only nodes with depth from root at least as low as $p'$ will have been rewired. So this rewiring is the first time any nodes on $T'_{p'}$ will have been rewired.

    The limited rewiring will occur when we add edge $(\mathtt{marked}_{T'}(p'),\mathtt{marked}_B(p))$ to the leaf-to-leaf tree. Let $u$ be the grandparent of $\mathtt{marked}_{T'}(p')$, and assume $u$ is an interior node. Suppose $u$ has two children $u_1$ and $u_2$ and $\mathtt{marked}_{T'}(p')\in T'_{u_1}$. By the left-to-right tree construction and since no rewiring has been done below $p'$ we know that $T_{v_2}$ will exactly have two leaf-to-leaf edges incident to it, $\{u,\mathtt{marked}_{T'}(v_2)\}$ and $\{x, \mathtt{marked}_{T'} (v_2)\}$ for some $x\in T'$. The rewiring is to delete the edge $\{x, \mathtt{marked}_{T'} (v_2)\}$ and add edge $\{x, v\}$. This rewiring will change the cost of the tree its in by at least $\frac{1}{5}+\frac{1}{6} - \frac{1}{4}-\frac{1}{5} = -\frac{1}{12}$. When we then append $B$ after this the increase changes in these last to nodes from $\frac{1}{5}+\frac{1}{6}$ to instead being $\frac{1}{6}+\frac{1}{7}-\frac{1}{12}$ which is enough to get the desired bound. 
    
    If $u$ does not have $2$ children, then $u$ has a budget of $1/3$ and this can be used instead when $B$ is appended. If a tree is appended at $p'$ again after $B$ is appended, the leaf-to-leaf edge added will be incident to $\mathtt{marked}_{T'}(p')$ and the same path that $B$ increased, this is a low cost, at most $1.8314814$

\end{proof}
  

\begin{lemma}
    Let $B$ be an extended binary tree rooted at vertex $p$, with $|P_{p,\mathtt{marked}_B(p)}| = 2$, that is appended to vertex $p'\in T'$. Then the new $H$-average of $T'$ will be at most $1.869047619$
\end{lemma}
\begin{proof}
    We are interested in the cases here that lead to $B$ having a cost greater than or equal to the stated bound. There are only so many cases cases
    
    \begin{enumerate}
   
        \item If $p'$ has two children that are leaves. $p$ has 3 children that are leaves. 1.875
        \item if $p'$ has two children that are leaves. $p$ has 2 children. not as bad as previous case
        \item if $p'$ has three children that are leaves. obviously not as bad as previous cases.
        \item $p'$ has 4 grandchildren. $B$ is two leavse
        \item $p'$ has more than 4 granchildren. $B$ is two leaves. 1.844444...
        \item $p'$ has more than 4 granchildren. $B$ is 3 leaves. even better
        \item $p'$ has 6 grandkids and $b$ is 3 leaves. charge to whole path you connect to. 
        \item $p'$ has 6 grandkids and has been used before. $B$ is 3 leaves. 1.869047619
     \end{enumerate}
\end{proof}


\begin{lemma}
    Let $B$ be an extended binary tree rooted at vertex $p$, with $|P_{p,\mathtt{marked}_B(p)}| = 1$, that is appended to vertex $p'\in T'$. Then the new $H$-average of $T'$ will be at most $1.885238$  
\end{lemma}  
\begin{proof}
    
\end{proof}
  
  
\begin{lemma}\label{lemma:decreasing-depth}
    The order of the trees we append is monotonically increasing with respect to distance from the root. 
\end{lemma}

\begin{algorithm}
    Let $T' = T_0$;\\
    Let $G' \coloneqq \mathtt{GenerateLeftToRightTree}(T')$;
    
    \For{each $B \in \mathcal{B}_1$}
    {
        $G(B) \coloneqq \mathtt{GenerateLeftToRightTree}(B)$;\\
        Set $\mathtt{marked}_1(root(B)) \coloneqq \ell_1(B)$.\\
        Set $\mathtt{marked}_2(root(B)) \coloneqq \ell_m(B)$.
    }
    
    \While{$(\mathcal{B}_1 \neq \emptyset)$}
    {
        Pick $(B,p') \in \mathcal{B}_1$ such that $p' \in T'$, and $p'$ is maximal amongst all such $p'\in T'$\\
        $\mathcal{B}_1 \coloneqq \mathcal{B}_1 \setminus \{(B,p')\}$.
        
        \If{$p' \in T_0$ and $w(p') =2$}
        {
            $G' \coloneqq G' \cup G(B) \cup \{(\ell_1(B), \mathtt{marked}_1(p'))\}$
        }
        
        \eIf{If $w(p')\geq 3$ but $p'$ has been used to append another tree before or $w(p')=2$ and $deg_{T'}(p') \geq 3$}
        {
            $G' \coloneqq G' \cup G(B) \cup \{(\ell_1(B), \mathtt{marked}_2(p'))\}$\\
            If $marked_2(p')$ has not been rewired, then rewire.
        }
        {
            $G' \coloneqq G' \cup G(B) \cup \{(\ell_1(B), \mathtt{marked}_1(p'))\}$\\
            If $marked_1(p')$ has not been rewired, then rewire.
        }
    }
    \Return{(T',G')}
\caption{Appending binary trees with $SP$-value at least $2$, one at a time}
\end{algorithm}
\label{alg:main-algorithm}
    

\paragraph{The Second Phase of the Algorithm.} Once we have run the first phase of the algorithm and appended every tree $B\in\mathcal{B}$ with $SP(B)\geq 2$, it remains to add the trees in $\mathcal{B}$ that possess a single Steiner node. In the first phase of the algorithm, we append the trees one by one and charge the increase in cost to the appended tree $B$. In this second phase we will instead append the remaining trees in groups and charge the increase to the whole group simultaneously. 
\begin{algorithm}
    \begin{enumerate}
        \item Input: $(T', G')$ from phase 1 of the algorithm
        \item While $(\mathcal{B} \neq \emptyset)$
        \begin{enumerate}
            \item Pick $(B_1,p'), (B_2,p'), \dots, (B_n,p')\in \mathcal{B}$, all trees in $\mathcal{B}$ that share a particular parent $p'$
            \item Set $\mathcal{B}\coloneqq \mathcal{B} \setminus \{(B_1,p'),(B_2,p'),\dots, (B_n,p')\}$
            \item Generate terminal-spanning trees $G_1,\dots,G_n$ for $B_1,\dots,B_n$ respectively
            \item Set $G' \coloneqq G'\cup \left(\cup_{i=1}^n G_n \right) \cup \left (\cup_{i=1}^n \{ \mathtt{marked}(p'),\mathtt{marked}(p_i)\}\right)$, where $p_i$ is the Steiner node of $B_i$
            \item Set $T' \coloneqq T' \cup \left(\cup_{i=1}^n B_n \right) \cup \left(\cup_{i=1}^n \{(p',p_i)\}\right)$
        \end{enumerate}
        \item Return $(T', G')$
    \end{enumerate}
\end{algorithm}



==> computing_terminal_spanning_tree.tex <==
%%%%%%%%%%%%%%%%% Appending binary trees to an existing tree %%%%%%%%%%%%%%%%% 
\section{Computing a terminal-spanning tree}
%In this section we show that the $H$-average of any tree $T$ is at most $1.94489$ by splitting the tree into a family of binary trees based on their marked paths. First, we will show that by ignoring certain nodes we can achieve a bound on the $H$-average of $1.872$, and then show that appending those ignored nodes leads to a bound of $1.94489$.

In this section, we give an upper bound on the average $H(w)$-value for any tree $T$ with the following property: if $N(R)$ is the set of Steiner nodes adjacent to the set of terminals $R$, then $T\setminus R$ is a tree and the set of leaves of $T\setminus R$ is equal to $N(R)$. We call the nodes of the set $N(R)$ the \emph{final} Steiner nodes of T.

Let $T = (V, E)$ be a tree, let $R \subseteq V$ be the set of terminals it contains, and let $F \subseteq V$ be the set of final Steiner nodes it contains. Our goal is to compute a terminal spanning tree that has a small $H$-average. Given the structure of the trees we are dealing with, and in order to simplify notation, we will instead compute a tree spanning the final nodes of the tree $T$. Any such tree directly corresponds to a terminal spanning tree as follows. For each final Steiner node $f \in F$, we arbitrarily pick one of the (at most) two terminals adjacent to $f$, which we denote as $\mathtt{rep}(f)$. Given a tree $T'$ that is a spanning tree on the final Steiner nodes, we can now generate a terminal spanning tree as follows:
\begin{itemize}
    \item we replace every edge $(f, f')$ of $T'$ with the edge $(\mathtt{rep}(f), \mathtt{rep}(f'))$,
    \item in case a final Steiner node $f$ has a second terminal $t$ adjacent to it besides $\mathtt{rep}(f)$, we also add the edge $(\mathtt{rep}(f), t)$ to the tree.  
\end{itemize}

It is easy to see that the $w$-values imposed by the tree spanning the final Steiner nodes and the corresponding terminal spanning tree are the same for all nodes except for the final Steiner nodes, where they differ by 1 in the case where a final Steiner node has two terminals adjacent to it. Thus, from now on, we only consider trees spanning the final Steiner nodes and we simply increase the corresponding $w$-value of each final Steiner node by $1$. For simplicity, we also assume that the given tree does not contain any terminals, and the task now reduces to computing a tree spanning the leaves of the tree.


The first step towards computing such a tree is to root the input tree $T$ at an arbitrary non-leaf node $r$. Thus, from now on we assume that $T$ is rooted. Given a rooted tree $T$, we will call the set of vertices with no children as \emph{leaves}; note that this allows the root to have degree $1$ without being a leaf, while other nodes that have degree $1$ are leaves. Reiterating, from now on we assume that we are given a tree $T$ rooted at a vertex $r$, where the set of final Steiner nodes is identical to the set of leaves of $T$.



Given a tree $T = (V, E)$ rooted at a vertex $r$, we introduce the following notation that we use throughout this section:
\begin{itemize}
    \item For every $x \in V$, $T_x$ denotes the subtree of $T$ ``hanging'' from the vertex $x$; in other words $T_x$ contains all the descendants of $x$, including $x$ itself.
    \item For every $u, v \in V$, $P_T(u,v)$ denotes the set of vertices in the unique path from $u$ to $v$ in $T$ (including $u$ and $v$).
    \item For every $x \in V$, $\mathtt{Child}_T(x) \subseteq V$ denotes the set of children of $x$.
    \item For every $x \in V$, $\mathtt{Sibling}_T(x) \subseteq V$ denotes the set of siblings of $x$, i.e., the set of vertices other than $x$ that have the same parent as $x$.
    \item For every $x \in V \setminus \{r\}$, $\mathtt{parent}_T(x)$ denotes the parent of $x$.
    \item $|T|$ denotes the number of nodes contained in $T$.
\end{itemize}

Throughout this section, we assume that both the root $r$ of $T$ and a ranking $\pi$ of the leaves of $T$ are fixed from the beginning and do not change throughout the execution of the algorithm; the reason that we need a ranking $\pi$ of the leaves will become clear in Section~\ref{sec:appending}. Given the rooted tree $T$ and an ordering $\pi$ of its leaves, we now introduce the concept of a \emph{marked} leaf.

\begin{definition}[Marked leaf]
Let $T = (V, E)$ be a tree, rooted at a vertex $r \in V$, and let $F \subseteq V$ be its set of leaves. Let $\pi: F \to [|F|]$ be a ranking of the leaves of $T$. Let $x \in V$, and $M_x \coloneqq \arg \min_{f \in F \cap T_x} \{|P_T(x,f)|\} \subseteq F \cap T_x$. Then, the marked leaf corresponding to $x$ is $\mathtt{marked}_T(x) \coloneqq \arg \min_{f \in M_x} \{\pi(f)\}$.
\end{definition}

We will sometimes skip the subscript and simply write $\mathtt{marked}(x)$ instead of $\mathtt{marked}_T(x)$, if the tree $T$ we are referring to is clear from the context. For a tree $T$, we also write $\mathtt{Marked}(T) \coloneqq \{f \in F: \exists x \in V \setminus F \textrm{ s.t. } \mathtt{marked}(x) = f\}$. Moreover, we define a total ordering $\prec$ over all rooted subtrees of $T$. More precisely, given a subtree $T_1$ rooted at $p_1$ and a subtree $T_2$ rooted at $p_2$, we write $T_1 \prec T_2$ if one of the following conditions is satisfied:
\begin{enumerate}
    \item $|P_{T_1}(p_1, \mathtt{marked}(p_1))| < |P_{T_2}(p_2, \mathtt{marked}(p_2))|$, or
    \item $|P_{T_1}(p_1, \mathtt{marked}(p_1))| = |P_{T_2}(p_2, \mathtt{marked}(p_2))|$ and $\pi(\mathtt{marked}(p_1)) < \pi(\mathtt{marked}(p_2))$.
\end{enumerate}


The rest of this section is organized as follows. We first consider the case of extended binary trees (see Definition~\ref{def:extended-binary-tree} in Section~\ref{sec:left-to-right-binary}), and construct a spanning tree of the leaves whose average $H$-value is bounded by $1.84$, and also has some additional properties that will be useful when dealing with the general case. In order to deal with arbitrary trees, we first decompose them into a family of extended binary trees; this decomposition is described in Section~\ref{sec:decomposition}. We then maintain a main tree, and use an iterative procedure to attach each binary tree to the main tree, one at a time, while maintaining a spanning tree on the leaves.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{``Left-to-Right'' Spanning Trees for Extended Binary Trees}\label{sec:left-to-right-binary}

In this section, we restrict our attention to rooted extended binary trees, defined as follows.
\begin{definition}[Extended Binary Tree]\label{def:extended-binary-tree}
    Let $T = (V, E)$ be a tree rooted at a vertex $r \in V$. Let $F \subseteq V$ be its set of leaves. $T$ is a rooted extended binary tree if for every vertex $x \in V \setminus F$, one of the following properties holds: (i) $|\mathtt{Child}_T(x)| \leq 2$, or (ii) $\mathtt{Child}_T(x) \subseteq F$ and $|\mathtt{Child}_T(x)| \leq 3$.
\end{definition}



We will now describe a procedure that produces a tree spanning the leaves of a rooted extended binary tree. Our procedure works in two steps. Given an extended binary tree $T$, in the first step we compute what we call a Left-to-Right tree spanning the subset $\mathtt{Marked}(T)$ of leaves. For that, we embed the rooted tree on the plane (in a specific way we will explain shortly), and then process the leaves, from left to right, and connect each pair of consecutive leaves with an edge. Once we are done with this step, we connect the leaves that were ignored, connecting each one of them with a single edge to its ``marked sibling''.

We now give some more details. Let $T = (V, E)$ be an extended binary tree rooted at $r \in V$, and let $F \subseteq V$ be its set of leaves. We first compute a spanning tree of $\mathtt{Marked}(T)$, as follows. We compute an ordering $(f_1, \ldots, f_m)$ of all the leaves in $\mathtt{Marked}(T)$, where $m = |\mathtt{Marked}(T)|$ and then, using this ordering we construct the spanning tree that contains the edges $(f_i, f_{i + 1})$, for every $i \in [m-1]$. Let $T' = T\left[(V \setminus F) \cup \mathtt{Marked}(T)\right]$. The procedure $\mathtt{GenerateLeftToRightOrdering}(T')$, described in Algorithm~\ref{alg:left-to-right-ordering}, generates such an ordering. Note that the procedure works for any rooted binary tree.

\begin{algorithm}[ht]
\If{$\mathtt{Child}_{T'}(r) = \emptyset$}{\Return $(r)$}

\If{$\mathtt{Child}_{T'}(r) = \{v\}$}{\Return $\mathtt{GenerateLeftToRightOrdering}(B'_v)$}

\tcp{Let $\mathtt{Child}_{T'}(r) = \{v_1, v_2\}$.}

$(f_1^{(1)}, \ldots, f_{m_1}^{(1)}) \leftarrow \mathtt{GenerateLeftToRightOrdering}(T'_{v_1})$

$(f_1^{(2)}, \ldots, f_{m_2}^{(2)}) \leftarrow \mathtt{GenerateLeftToRightOrdering}(T'_{v_2})$

\eIf{$T'_{v_1} \prec T'_{v_2}$}
        {\Return $(f_1^{(1)}, \ldots, f_{m_1}^{(1)}, f_{m_2}^{(2)}, f_{m_2 - 1}^{(2)}\ldots, f_{1}^{(2)})$}
        {
        \Return $(f_1^{(2)}, \ldots, f_{m_2}^{(2)}, f_{m_1}^{(1)}, f_{m_1 - 1}^{(1)}\ldots, f_{1}^{(1)})$
        }
\caption{The $\mathtt{GenerateLeftToRightOrdering}(T')$ procedure}
\label{alg:left-to-right-ordering}
\end{algorithm}


We now present the procedure $\mathtt{GenerateLeftToRightTree}(T)$, described in Algorithm~\ref{alg:left-to-right-tree}, that works for any rooted extended binary tree.


\begin{algorithm}[ht]

Let $T' \leftarrow T[(V \setminus F) \cup \mathtt{Marked}(T)]$

$(f_1, \ldots, f_m) \leftarrow \mathtt{GenerateLeftToRightOrdering}(T')$

$E' \leftarrow \emptyset$

\For{$i = 1, \ldots, m-1$}
         {$E' \leftarrow E' \cup \{(f_i, f_{i+1})\}$}
         
\For{$i = 1, \ldots, m$}
        {\For{$f' \in \mathtt{Sibling}(f_i)$}
            {$E' \leftarrow E' \cup \{(f_i, f')\}$}
        }
        
$G(T) \leftarrow (F, E')$

\Return $G(T)$

\caption{The $\mathtt{GenerateLeftToRightTree}(T)$ procedure}
\label{alg:left-to-right-tree}
\end{algorithm}




We now present some useful lemmas about the trees generated by our procedure. The first one deals with the case where the input tree is a path, the second one deals with the case of a binary tree, and the third one deals with the case of an extended binary tree.

\begin{lemma}\label{lemma:left-to-right-single-path}
Let $T$ be a binary tree rooted at $r$ that is a path, i.e., there is exactly one leaf $f$ in $T$. Then, the $\mathtt{GenerateLeftToRightTree}(T)$ procedure produces a tree with a single vertex and no edges, such that $w(f) = 1$, and $w(x) = 0$ for every $x \in B \setminus \{f\}$.
\end{lemma}
The proof of the above lemma is immediate and, thus, omitted.

\begin{lemma}\label{lemma:left-to-right-properties-skeleton}
Let $T = (V, E)$ be a binary tree that is not a path, rooted at a vertex $r \in V$, and let $F \subseteq V$ be its set of leaves. Let $(f_1, \ldots, f_m)$ be the output of the $\mathtt{GenerateLeftToRightOrdering}(T)$ procedure, and let $G(T)$ be the corresponding tree. Let $w: V \to \mathbb{N}_{\geq 0}$ be the $w$-value implied by $G(T)$. If $|\mathtt{Child}_T(r)| = 1$, let $r'$ be the first descendant of $r$ that has two children, otherwise let $r' \coloneqq r$. Let $v_1$ and $v_2$ be the two children of $r'$. Then, the following properties are satisfied:
\begin{enumerate}
    \item $w(x) = 0$ for every ancestor $x$ of $r'$, if any.
    \item $w(r') = 1$.
    \item $f_1 = \mathtt{marked}(r')$. Moreover, assuming wlog that $f_1 \in T_{v_1}$, then $f_m = \mathtt{marked}(v_2)$.
    \item $w(x) = |\mathtt{Child}_T(x)|$, for every $x \in \left(P_T(r',f_1) \cup P_T(r', f_m) \right) \setminus \{r', f_1, f_m\}$.
    \item $w(x) = |\mathtt{Child}_T(x)| + 1$, for every $x \notin P_T(r',f_1) \cup P_T(r',f_m) \cup P_T(r, r') \cup \{f_1, \ldots, f_m\}$.
    \item $w(f_1) = w(f_m) = 2$.
    \item $w(f_i) = 3$, for every $i \in \{2, \ldots, m-1\}$.
\end{enumerate}
\end{lemma}
\begin{proof}
We use induction on the number of vertices $|T|$ of $T$. If $|T| = 3$, which is the minimal case for which a tree contains a vertex that has two children, then the statement holds trivially. So, suppose that it holds for all trees of size smaller than $n \geq 4$, and let $|T| = n$. If $r$, the root of $T$ has only one child $v$, then the statements hold by the induction hypothesis applied on the tree $T_v$; clearly we have $w(r) = 0$ in this case.

Suppose now that $r$ has two children $v_1$ and $v_2$. We use the induction hypothesis on the trees produced by the recursive calls on $T_{v_1}$ and $T_{v_2}$. The only connection made to join these two trees is the addition of the edge $(f_{m_1}^{(1)}, f_{m_2}^{(2)})$. It is easy to see that $w(x) = 0$ for every $x \in P_T(r,r') \setminus \{r'\}$, and so property (1) is satisfied. It is also easy to see that property (2) is satisfied, since there is only one path passing through $r$, the one connecting $f_{m_1}^{(1)}$ with $f_{m_2}^{(2)}$. Property (3) also holds due to induction hypothesis and the final choice made by the algorithm. To show property (4), we note that the only vertices of the set $P_T(r', f_1^{(1)}) \cup P_T(r', f_1^{(2)}) \setminus \{r', f_1^{(2)}, f_2^{(2)}\}$ that can are affected by the addition of the edge $(f_{m_1}^{(1)}, f_{m_2}^{(2)})$ are the vertices on the path from $v_1$ down to its first descendant that has two children, if there is such a path, and similarly, the vertices on the path from $v_2$ down to its first descendant that has two children, if there is such a path. All such vertices, if any, by the induction hypothesis had $w$-value equal to $0$, which now becomes $1$. We conclude that proeprty (4) is satisfied.

Using the induction hypothesis, property (6) is also immediate since we either have that $f_1^{(1)}$, and similarly $f_1^{(2)}$, is not affected by the addition of the edge $(f_{m_1}^{(1)}, f_{m_2}^{(2)})$ or the subtree $T_{v_1}$, and similarly $T_{v_2}$ is a single path. In any case, the statement holds by the induction hypothesis and Lemma~\ref{lemma:left-to-right-single-path}. To prove property (5), we note that if there are vertices that are affected by the addition of the edge $(f_{m_1}^{(1)}, f_{m_2}^{(2)})$ which are not part of $P_T(r', f_1) \cup P_T(r', f_m) \cup P_T(r, r') \cup \{f_1, \ldots, f_m\}$, then these vertices must belong to a subpath of $P_T(v_1, f_{m_1}^{(1)}) \cup P_T(v_1, f_{m_2}^{(2)})$. By the induction hypothesis, any such vertex $x$ had $w$-value $w(x) = |\mathtt{Child}(x)|$ before the addition of $(f_{m_1}^{(1)}, f_{m_2}^{(2)})$, and so it now has $w'(x) = |\mathtt{Child}(x)| + 1$. For the rest of the vertices are not affected by the addition of this edge, and so using the induction hypothesis, the statement holds. Finally, property (7) is immediate by the induction hypothesis.
\end{proof}


Using the above lemma, we can now easily deduce the properties of the tree generated by the  $\mathtt{GenerateLeftToRightTree}(T)$ procedure that works for any extended rooted binary tree $T$.
\begin{lemma}\label{lemma:extended-binary-tree-properties}
Let $T = (V, E)$ be an extended binary tree rooted at $r$, and let $F \subseteq V$ be its set of leaves. Let $T' = T[(V \setminus F) \cup \mathtt{Marked}(T)]$, and let $(f_1, \ldots, f_m)$ be the ordering produced by the $\mathtt{GenerateLeftToRightOrdering}(T')$ procedure. Let $G(T)$ be the tree generated by the $\mathtt{GenerateLeftToRightTree}(T)$ procedure. Let $F = \{f_1, \ldots, f_m\} \cup F_0$ be the set of leaves of $T$. Then, the first 5 properties of Lemma~\ref{lemma:left-to-right-properties-skeleton} hold. For the set of leaves $F$, we have $w(f) = |\mathtt{Sibling}_T(f_i) \cap F| + 3$ for every $i \in \{2, \ldots, m-1\}$, $w(f_i) = |\mathtt{Sibling}_T(f_i) \cap F| + 2$ for $i \in \{1,m\}$ and $w(f) = 2$ for every $f \in F_0$.
\end{lemma}


The above lemma can now be used to get a bound on the average $H(w)$-value implied by the generated leaf-spanning tree. More precisely, we prove the following lemma.
\begin{lemma}\label{lemma:extended-binary-tree-bounds}
Let $T=(V, E)$ be an extended binary tree rooted at $r$, and let $F \subseteq V$ be its set of leaves. Let $G(T)$ be the tree generated by the $\mathtt{GenerateLeftToRightTree}(T)$ procedure, and let $w: V \to \mathbb{N}_{\geq 0}$ be the corresponding $w$ function. Then, we have $\E[H(w(v))] < 1.84$.
\end{lemma}
\begin{proof}
In case $T$ is a path, then the statement is immediate. Thus, we assume that $T$ is not a path. Let $(f_1, \ldots, f_m) = \mathtt{GenerateLeftToRightOrdering}(T')$, where $T' = T[(V \setminus F) \cup \mathtt{Marked}(T)]$. By Lemma~\ref{lemma:extended-binary-tree-properties}, the only vertices of $T$ that can have a $w$-value strictly greater than $3$ are the leaves $\{f_1, \ldots, f_m\}$, and the parents of the leaves $\{f_2, \ldots, f_{m-1}\}$.

Let $f_i$, $i \in \{2, \ldots, f_{m-1}\}$, be a leaf that satisfies $w(f_i) > 3$. In such a case, we have $\mathtt{Sibling}_T(f_i) \subseteq F$ and $|\mathtt{Sibling}_T(f_i)| \in \{1, 2\}$. Let $p \coloneqq \mathtt{parent}_T(f_i)$. We do some case analysis:
\begin{itemize}
    \item $\mathtt{Sibling}_T(f_i) = \{f\}$. In this case, $w(f_i) = 4$ and $w(p) = 3$. This means that
        \begin{align*}
            H(w(f_i)) + H(w(f)) + H(w(p)) &= H(4) + H(2) + H(3) = 3 H(3) - \frac{1}{12}
        \end{align*}
    \item $\mathtt{Sibling}_T(f_i) = \{f, f'\}$. In this case, $w(f_i) = 5$ and $w(p) = 4$. This means that
    \begin{align*}
            H(w(f_i)) + H(w(f)) + H(w(f')) + H(w(p)) &= H(5) + H(2) + H(2) +  H(4)\\
                                &= 4 H(3) + \frac{1}{30} = 4 \left(H(3) + \frac{1}{120} \right).
    \end{align*}
\end{itemize}

We now turn to the case of $f_i$ where $i \in \{1,m\}$. We only consider $f_1$, since the analysis for $f_m$ is identical. If $w(f_1) > 3$, then we must have $\mathtt{Sibling}_T(f_1) = \{f, f'\} \subseteq F$. In such case, $p \coloneqq \mathtt{parent}_T(f_1)$ has $w(p) = 3$, and so we get that
\begin{align*}
    H(w(f_i)) + H(w(f)) + H(w(f')) + H(w(p)) &= H(4) + H(2) + H(2) + H(3)\\
                                             &= 4 H(3) - \frac{5}{12} = 4 \left(H(3) - \frac{5}{48}\right).
\end{align*}

Given that all other vertices have a $w$-value of at most $3$, the above already implies that $\E[H(w(v))] = \frac{1}{|V|} \sum_{v \in V} H(w(v)) \leq H(3) + \frac{1}{120} < 1.842$.


In order to get a slightly improved bound, we note that the only case where the average can go above $H(3)$ is when $f_i$, $i \in \{2, \ldots, m-1\}$, has 2 siblings. Let $Z = \{x \in V: |\mathtt{Child}_T(x)| = 3\} \setminus \{\mathtt{parent}_T(f_1),\mathtt{parent}_T(f_m)\}$. Note that $Z$ is necessarily a subset of $\{p \in V: \exists i \in\{2, \ldots, m-1\} \textrm{ s.t. }p = \mathtt{parent}_T(f_i)\}$. Thus, $z = |Z| \leq m-2$. Suppose now that we remove the set $\bigcup_{p \in Z}\mathtt{Child}_T(z)$ from the tree. What is left is a rooted binary tree where every node in $Z$ appears as a leaf; note that $f_1$ and $f_m$ also appear as leaves of this tree, and do not belong to $Z$. Thus, the number of nodes that do not belong to the set $\bigcup_{p \in Z}\mathtt{Child}_T(p) \cup Z$ must be at least $z - 1 + 2 > z$. This implies that
\begin{equation*}
    \E[H(w(v))] = \frac{1}{|V|} \sum_{v \in V} H(w(v)) < \frac{z H(3) + 4z (H(3) + \frac{1}{120})}{5z} = H(3) + \frac{1}{150} = 1.84.
\end{equation*}
\end{proof}


Before proceeding to describe how we decompose any tree into a family of extended binary trees, we introduce some further notation for extended binary trees. Let $T = (V, E)$ be an extended binary tree rooted at a vertex $r$ that is not a path, and let $F \subseteq V$ be its set of leaves. Let $(f_1, \ldots, f_m) = \mathtt{GenerateLeftToRightOrdering}(T')$, where $T' = T[(V \setminus F) \cup \mathtt{Marked}(T)]$. Then, in case $m > 1$, we define $\mathtt{marked}_T^{(1)}(r) \coloneqq f_1$ and $\mathtt{marked}_T^{(2)}(r) \coloneqq f_m$.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
\subsection{Decomposing into a family of Extended Binary Trees}\label{sec:decomposition}

In this section, we describe a procedure that takes as input a tree $T$ rooted at a vertex $r$ and partitions it into a family of rooted extended binary trees. More precisely, the output is a pair $(T_0, \mathcal{B})$, where $T_0$ is a rooted extended binary tree containing $r$, and $\mathcal{B}$ is a set of pairs $(B, p')$, where each $B$ is a rooted extended binary tree, rooted at a vertex $p$, and $p' \notin B$ is a vertex that is not part of the tree $B$, such that $p' = \mathtt{parent}_T(p)$.

Intuitively, the procedure, described in Algorithm~\ref{alg:partition-into-binary-trees}, computes an extended binary tree $T_0$ containing the root by considering the subtrees rooted at the children of $r$ and selecting the two ``smallest'' ones, according to the ordering $\prec$ (or three of them, in case they are all leaves). The remaining forest is then decomposed recursively.

\begin{algorithm}[ht]
\If{$|T| \leq 1$}{\Return $(T, \emptyset)$}

Let $\mathtt{Child}_T(r) = \{v_1, \ldots, v_k\}$, for $k \in \mathbb{N}_{\geq 1}$, and wlog assume that $T_{v_1} \prec T_{v_2} \prec \ldots \prec T_{v_k}$.

\If{$|T_{v_k}| = 1$}
    {
        $T_0 \leftarrow \{(r, v_i): i \in \{1, \ldots, \min\{3,k\}\}\}$
        
        $\mathcal{B} \leftarrow \{(\{v_i\}, r): i \in \{4, \ldots, k\}\}$
        
        \Return $(T_0, \mathcal{B})$       
        
    }



    \For{$i = 1, \ldots, k$}
        {
        $(B_i, \mathcal{B}_i) \leftarrow \mathtt{PartitionIntoBinaryTrees}(T_{v_i})$
        }           
         
        $\mathcal{B} \leftarrow \left(\bigcup_{i = 1}^k \mathcal{B}_i \right) \cup \left\{(B_i, r): i \in \{3, \ldots, k\} \right\}$
        
    
    \eIf{$k \geq 2$}{$T_0 \leftarrow \{(r,v_1), (r, v_2)\} \cup B_1 \cup B_2$}
    {$T_0 \leftarrow \{(r, v_1)\} \cup B_1$}
 
\Return $(T_0, \mathcal{B})$;

\caption{The $\mathtt{PartitionIntoBinaryTrees}(T)$ procedure.}
\label{alg:partition-into-binary-trees}
\end{algorithm}

It is now easy to prove the following lemma.
\begin{lemma}
    Given a tree $T$, Algorithm~\ref{alg:partition-into-binary-trees} partitions $T$ into a family of rooted extended binary trees.
\end{lemma}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\input{./appending_binary_trees.tex}

==> k_restricted_node_steiner.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{$k$-restricted (unweighted) TAP-Node-Steiner Ratio}

In this section, we are interested in $k$-restricted Node Steiner trees.
\begin{definition}[$k$-restricted Node Steiner Tree]
Given is a Node Steiner Tree instance. A component is a tree where every terminal contained in it is a leaf. A $k$-restricted Steiner tree is a collection of components, with at most $k$ terminals each, whose union induces a feasible Steiner tree. The cost of a $k$-restricted Steiner tree is the sum of the costs of its components, counting duplicated vertices with their multiplicity.
\end{definition}

We will show that, by losing a small $\varepsilon$-factor, we can restrict our attention to $k$-restricted Steiner trees. More precisely, the main theorem of this section is the following.
\begin{theorem}\label{thm:k-restricted-decomp}
Let $G=(C \cup L, F)$ be a TAP-Node-Steiner-Tree instance, and let $OPT$ be its optimal value. Then, for any integer $m \geq 1$, there exists a $k$-restricted Steiner tree $Q(k)$, for $k = 2^m$, whose cost satisfies
\begin{equation*}
    cost(Q(k)) \leq \left(1 + \frac{4       }{\log k}\right) OPT. 
\end{equation*}
\end{theorem}
Before proving the above theorem, we stress that we crucially use all the properties stated in Observation~\ref{obs:properties}, as well as the following observations and lemmas.
\begin{observation}\label{obs:lower-bound}
Let $OPT$ be the optimal cost of a TAP-Node-Steiner-Tree instance with $t$ terminals. Then, we have $OPT \geq \frac{t}{2}$.
\end{observation}

\begin{definition}
A rooted binary tree is called regular if every non-leaf node has exactly $2$ children.
\end{definition}

\begin{lemma}\label{lemma:map}
    For any regular binary tree, there exists a one-to-one mapping $f$ from internal nodes to leaves, such that
    \begin{itemize}
        \item for any internal vertex u, $f(u)$ is a descendent of $u$, and
        \item all tree paths from $u$ to $f(u)$ are pairwise edge disjoint, and internally they are also node disjoint.
    \end{itemize}
\end{lemma}
The proof of the above lemma is given in Appendix~\ref{appendix:proofs}.

\begin{lemma}\label{lemma:high-degree-vertices-vs-leaves}
Let $T = (V, E)$ be a tree with $t$ leaves. Then, we have $\sum_{v\in V : d(v) \geq 3} (d(v) - 2) \leq t$.
\end{lemma}
The proof of the above lemma is standard, and is given in Appendix~\ref{appendix:proofs}.



We are now ready to prove Theorem~\ref{thm:k-restricted-decomp}.

\begin{proof}[Proof of Theorem~\ref{thm:k-restricted-decomp}]
We begin with an optimal solution $Q$ of cost $OPT$ to our TAP-Node-Steiner-Tree instance and modify it as described in Xu et al.~\cite{xu2010approximations} to get a new tree $Q^+$ of equal cost. More precisely, we first create a dummy Steiner node of zero weight in the middle of an edge that serves as the root of the tree; thus, from now on $Q$ will be a rooted tree. For each Steiner node $v$ that has at least three children, we expand $v$ into a binary tree by using duplicate nodes of zero weight such that every node in the resulting tree has at most two children. The following lemma, whose proof is straightforward and thus omitted, shows that the number of auxiliary nodes is proportional to the degree of the node that is modified.

\begin{lemma}\label{lemma:degree}
Let $v$ be a node of $Q$ with at least three children. Then, if we apply the transformation described above to $v$, we get a new tree that contains $d(v)-3$ extra auxiliary nodes, where $d(v)$ is the degree of $v$.
\end{lemma}%

We can repeatedly apply the transformation described above, and we get a new tree $Q^+$ where every Steiner node has at most two children. This new tree $Q^+$ has at most
\begin{equation*}
    n + \sum_{v \in Q: d(v) \geq 4}(d(v) - 3) \leq n + 2(n-1) = 3n - 2
\end{equation*}
vertices, where $n$ is the number of vertices of the rooted tree $Q$. Finally, for any non-leaf node different from the root that has degree $2$, we add a dummy terminal as a child, and we end up with a regular node weighted binary tree (where only Steiner nodes have weight), which, by slightly abusing notation, we call $Q^+$. 

We now label the Steiner nodes of $Q^+$ with labels $\{0,\dots, m-1\}$ as follows; we stress that the labeling and the arguments used closely follow the techniques of Borchers and Du~\cite{DBLP:journals/siamcomp/BorchersD97}. We first clarify some terminology. We will say that the root is at the $0^{th}$ layer of $Q^+$, the children of the root are at the $1^{st}$ layer, and so on. We label the root with $0$, the $1^{st}$ layer of nodes with $1$, and so on until the $(m-1)^{th}$ layer. We then repeat the labelling with label $0$, starting from layer $m$. More precisely, the Steiner nodes on layer $i$ get the label $i \mod m$. We obviously have the property that any $m$ consecutive layers have different labels.

For each label $j \in \{0, \ldots, m-1\}$, we will define a feasible $k$-restricted Steiner tree $Q_j^+$. We only explicitly define its components; the tree $Q_j^+$ is simply the union of these components and its cost is the sum of the costs of its components. For a fixed label $j$, each component of $Q_j^+$ is rooted at either the root of $Q^+$ or a Steiner node with label $j$. Let $v$ be a Steiner node labelled with $j$. We define the component rooted at $v$ as follows: $v$ connects with paths in $Q^+$ to the first vertices below $v$ that are also labelled by $j$; call these vertices \emph{intermediate leaves}. Then for an intermediate leaf $u$, the component connects $u$ to $f(u)$ via a unique path $p(u)$, as defined in Lemma~\ref{lemma:map}. If there is a path below $v$ to a leaf of $Q^+$ that does not contain a node with label $j$, then that path is also in the component. The component of $Q_j^+$ that is rooted at the root of $Q^+$ is constructed in a similar way; we stress that every $Q_j^+$ contains a component rooted at the root of $Q^+$ (even if $j > 0$). 

\begin{lemma}
Each component of $Q_j^+$ has at most $k$ terminals.
\end{lemma}
\begin{proof}
It is clear that a component has at most $2^m$ intermediate leaves by the labelling procedure, and thus at most $2^m$ leaves connected by paths from these intermediate leaves. If there is a direct component-root-to-leaf path, then the leaf must be no more than $m$ layers below the component root. So, the total number of leaves for any component is at most $2^m = k$.
\end{proof}



\begin{lemma}\label{lemma:feasible}
Let $j \in \{0, \ldots, m-1\}$. The tree $Q_j^+$, as defined through its components above, is a feasible $k$-restricted Steiner tree.
\end{lemma}
\begin{proof}
To see this, we only need to look at the part of each component that connects a vertex $v$ labelled as $\ell$ to its intermediate leaves. It is easy to see that the union of all these components, along with the component rooted at the root of $Q^+$, partition $Q^+$, and so $Q_j^+$ is indeed a feasible $k$-restricted Steiner tree.
\end{proof}

Given a $k$-restricted Steiner tree $Q_j^+$ of $Q^+$, we now explain how to construct a $k$-restricted Steiner tree $Q_j$ of $Q$. For any component $B$ of $Q_\ell^+$ we construct a component $B'$ in $Q$ by contracting every expanded node and removing any dummy terminals and the root. Clearly $B'$ still has at most $k$ terminals, and thus the union of of these components of $Q$ is a $k$-restricted Node Steiner Tree, which we denote as $Q_j$. For the final step of our argument, we require the following observation about the $k$-restricted trees that will be useful in bounding the optimal cost.

\begin{observation}\label{obs1}
Consider the $k$-restricted Steiner trees $Q_0^+, \ldots, Q_{m-1}^+$ of $Q^+$, as defined above, and their corresponding components. Any non-root Steiner node appears as an intermediate leaf in exactly one component of exactly one such Steiner tree.
\end{observation}

Using this observation we will now find a bound on the sum $\sum_{j = 0}^{m-1}cost(Q_j)$. For that, we consider a Steiner node $v$ of $Q$. We first note that $v$ has $d(v) - 2$ ``copies" in $Q^+$. By Observation~\ref{obs1}, each such copy appears as an intermediate leaf, and thus, counted twice, in exactly one component of exactly one Steiner tree among $Q_0^+, \ldots, Q_{m-1}^+$. Finally, each such copy can appear at most one more time as an internal node of a path from an intermediate leaf to a leaf (as implied by Lemma~\ref{lemma:map}). Thus, $v$ appears at most $2(d(v) - 2) + m$ times in the sum $\sum_{j = 0}^{m-1}cost(Q_j)$. Let $S$ denote the set of Steiner nodes of $Q$, $S_2 = \{s \in S: d(s) = 2\}$ and $S_{\geq 3} = \{ s \in S: d(s) \geq 3\}$. Note that $S = S_2 \cup S_{\geq 3}$. Let $t$ be the number of terminals. We have
\begin{align*}
    \sum_{j = 0}^{m-1}cost(Q_j) &= m |S| + 2\sum_{s \in S} (d(s)-2)\\
                                &= m |S| - 4|S|+ 2\sum_{s \in S} d(s) \\
                                &= (m-4) |S| + 2\sum_{s \in S_2} d(s) + 2\sum_{s \in S_{\geq 3}} d(s)\\
                                &\leq (m-4) |S| + 4 \left(|S| - |S_{\geq 3} \right)  + 2\sum_{s \in S: d(s) \geq 3} d(v)\\
                                &= m \cdot OPT + 2\sum_{s \in S_{\geq 3}} (d(s) - 2)\\
                                &\leq m \cdot OPT + 2t\\
                                &\leq m \cdot OPT + 4OPT\\
                                &= (m+4)OPT,
\end{align*}
where in the above derivations we used Observation~\ref{obs:lower-bound} and Lemma~\ref{lemma:high-degree-vertices-vs-leaves}.

Thus, there exists a label $j \in \{0, 1, \ldots, m-1\}$ such that
\begin{equation*}
    cost(Q_j) \leq \left(1 + \frac{4}{\log k} \right) OPT.
\end{equation*}




\begin{comment}

of $Q^+$ with label $j$ and can count how much $v$ contributes to $\sum_{j = 0}^{m-1}cost(Q_j)$ by looking at the following three cases.

%We would now like to bound the cost difference $c(Q_l) - c(Q)$. That is, we want to compute the amount of Steiner nodes over-counted by $Q_l$. We consider the components on $Q^+$. For each internal node $v$ with label $l$ of $Q^+$ there are three cases to consider 
\begin{enumerate}
    \item  $v$ appears as an internal node $u$ of the path $p(v)$ provides cost at most $1$.
    \item If $v$ is a duplicate node, then the node $u$ that it duplicates provides cost 1.
    \item if $v$ is not a duplicate node, then $v$ provides cost 1.
\end{enumerate}

The nodes that fall under case 1 provide a total of at most $w(Q)$ cost to $\sum_{l = 0}^{m-1}(cost(Q_l)-cost(Q))$. This is because a node $u$ is charged when it is an internal node of a path $p(v)$. By Lemma \ref{lemma:map} we know that $u$ is an internal node of exactly one path $p(v)$ and we know by our labelling scheme that $p(v)$ is only part of one component; thus $u$ provides only a cost of 1 under case 1, and thus case 1 provides a cost of at most $w(Q)$.

Recall Lemma \ref{lemma:degree}, which says that the transformation of a node with at least three children creates $d(v) - 2$ nodes out of the original node. A node that isn't the root of $Q^+$ is the root of exactly 1 component by Observation \ref{obs1} and thus only charges 1 cost to case 3, and charges a cost of $d(v)-3$ to case 2. 

Let $S$ be the Steiner nodes of $Q$. For label $d$ minimizing $c(Q_d) - c(Q)$ we have
\begin{equation*}
    c(Q_d) - c(Q) \leq \frac{1}{m} \sum_{\ell = 0}^{m-1}(cost(Q_\ell)-cost(Q)) \leq \frac{1}{m}\sum_{v\in S}(1 + d(v)-2),
\end{equation*}
which gives
\begin{align*}
cost(Q_d) &\leq cost(Q) + \frac{1}{m}\sum_{v\in S}(d(v)-1) = opt\left(1 - \frac{1}{\log k}\right) + \frac{1}{\log k}\sum_{v\in S}d(v)\\
       &= opt\left(1 - \frac{1}{\log k}\right) + \frac{1}{\log k}\left (\sum_{v\in S : d(v) \geq  3}d(v) + \sum_{v\in S : d(v) = 2}d(v) \right)
\end{align*}
Using Observation~\ref{obs:lower-bound} and Lemma~\ref{lemma:high-degree-vertices-vs-leaves} we get that
\begin{align*}
    c(Q_d) &\leq opt\left(1 - \frac{1}{\log k}\right) + \frac{1}{\log k}\left (3t + \sum_{v\in S: d(v) = 2}d(v) \right)\\ 
    & \leq opt\left(1 - \frac{1}{\log k}\right) + \frac{6opt + 2|S|}{\log k}\\ 
    & \leq opt\left(1 - \frac{1}{\log k}\right) + \frac{8opt}{\log k}\\ 
    &= opt\left(1 + \frac{7}{\log k} \right).
\end{align*}
\end{comment}


\end{proof}




==> k_steiner_ratio_edge_case_writeup.tex <==
\section{k-Steiner Ratio with unit edge weights}

Throughout, we assume that we work on a metric instance, i.e., the underlying graph is a complete undirected graph with edge lengths $c: E \to \mathbb{R}_{\geq 0}$ that satisfy the triangle inequality. We also assume that $k = 2^r$, for some positive integer $r$; clearly, $r = \log k$.

\begin{definition}
A rooted binary tree is called regular if every non-leaf node has exactly $2$ children.
\end{definition}


\begin{lemma}\label{lemma:map1}
    For any regular binary tree, there exists a one-to-one mapping $f$ from internal nodes to leaves, such that
    \begin{itemize}
        \item for any internal vertex u, $f(u)$ is a descendent of $u$
        \item all tree paths from $u$ to $f(u)$ are edge disjoint
    \end{itemize}
\end{lemma}

\textcolor{red}{What is the canonical way of defining such a map?}\\


As proved by Al Borchers and Ding-Zhu Du, when it comes to the $k$-Steiner ratio, we only need to focus on the case where the optimal Steiner tree $T$ is a weighted regular binary tree, where every terminal is a leaf. More precisely, we assume that $T$ is a full Steiner tree solution; that is, every leaf is a terminal. We add zero cost edges and dummy nodes so that every Steiner node has degree exactly three. We then add a dummy node in the middle of an edge to create a root % should the weight be put on one of the two edges created?
and call this rooted tree $T'$. Note that since we only added dummy nodes and zero cost edges, the cost of the edges in $T'$ is equal to the cost of $T$.

We then label the Steiner nodes of $T'$ in the following way with labels $\{0,\dots, r-1\}$. We label the first layer of nodes (the root) $0$, the second layer of nodes $1$, and so on until the $r^{th}$ layer, then repeat the labelling with label $0$. So the Steiner nodes on layer $i$ are labelled $(i-1)\mod r$. We obviously have the property that any $r$ sequential layers have different labels.

For each label $l$, we will define a feasible $k$-restricted Steiner tree $T_l$. We only explicitly define its components; the tree $T_l$ is simply the union of these components. We fix a label $l$. Each component of $T_l$ is rooted at either the root of $T'$ or a Steiner node labelled by $l$. Let $v$ be a vertex labelled with $l$. We define the component rooted at $v$ as follows: $v$ connects by paths in $T'$ to the first vertices below $v$ that are also labelled by $l$; call these vertices \emph{intermediate leaves}. Then for an intermediate leaf $u$, the component connects $u$ to $f(u)$ by the path $p(u)$, as defined in Lemma~\ref{lemma:map1}. If there is a path below $v$ to a leaf of $T'$ that does not have a node with label $l$, then that path is also in the component. The component of $T_l$ that is rooted at the root of $T'$ is constructed in a similar way.

\begin{lemma}
Each component of $T_l$ has at most $k$ terminals.
\end{lemma}
\begin{proof}
It is clear that a component has at most $2^r$ intermediate leaves by the labelling procedure, and thus at most $2^r$ leaves connected by paths from these intermediate leaves. If there is a direct component-root-to-leaf path, then the leaf must be no more than $r$ layers below the component root. So, the total number of leaves for any component is at most $2^r = k$.
\end{proof}


\begin{lemma}\label{lemma:feasible}
Let $l \in \{0, \ldots, r-1\}$. The tree $T_l$, as defined through its components above, is a feasible Steiner tree.
\end{lemma}
\begin{proof}
To see this, we only need to look at the part of each component that connects a vertex $v$ labelled as $l$ to its intermediate leaves. It is easy to see that the union of all these components, along with the component rooted at the root of $T'$, partition $T'$, and so $T_l$ is indeed a feasible Steiner tree.
\end{proof}

\begin{observation}\label{obs1}
Consider the Steiner trees $T_0, \ldots, T_{r-1}$, as defined above, and their corresponding components. Any non-root Steiner node appears as an intermediate leaf in exactly one component of exactly one such Steiner tree.
\end{observation}

For any $l \in \{0, \ldots, r-1\}$, we define
\begin{equation*}
    L_l = \sum_{\substack{\text{$u \in T'$: $u$ is an} \\ \text{intermediate leaf in $T_l$}}} c(u,f(u)).
\end{equation*}
By Observation~\ref{obs1}, any non-root Steiner node is an intermediate leaf exactly once, so we have
\[
    L_0+\dots +L_{r-1} \leq c(T') = c(T)
\]
since the paths are edge disjoint by Lemma~\ref{lemma:map}. Furthermore, by a direct averaging argument, there is a label $d \in \{0, \ldots, r-1\}$ such that 
\[
    rL_d \leq L_0+\dots +L_{r-1},
s\]
which implies that there exists a label $d$ such that $L_d \leq \frac{c(T)}{r}$. Thus, Lemma~\ref{lemma:feasible} and its proof imply that the cost of the feasible $k$-restricted Steiner tree $T_d$ is
\[
    c(T_d) = C(T') + L_d \leq \left(1 + \frac{1}{r}\right)c(T) = \left (1 + \frac{1}{\log k}\right)c(T)
\]


\subsection{M bounded costs}

==> original_nutov_proof.tex <==
\subsection{Proof of Theorem~\ref{cor:approx-preserve-block}}\label{appendix:approx-preserve-block}
In this section we outline the reduction from a Block-TAP instance $(G = (V, E_G),L)$ to CA-Node-Steiner-Tree that was described by Nutov \cite{nutov20202nodeconnectivity}. The result of the reduction is intuitively similar to the reduction from \cite{DBLP:conf/stoc/Byrka0A20}, except the graph we construct for the Node-Steiner-Tree instance uses a subset of $E_G$ instead of a subset of $V$ as terminals. Edges that are incident to leaves in $V$ will be referred to as \emph{leaf-edges} for simplicity, and will eventually serve as our terminals. Now we can define our reduction to a Node-Steiner-Tree instance.

\begin{definition}
    Given a tree $G = (V,E_G)$, and a set of links $L$ on $V$, the \emph{$(L,E_G)$-incidence graph} is the graph with node set $L\cup E_G$ and edge set $\{\ell e : e\in G_{\ell}, \ell \in L\}$, where $G_{\ell}$ is the unique path on $G$ from the two endpoints of $\ell$. We let $E_G$ be the set of terminals of this graph, and $\ell \in L$ be the Steiner nodes. We can define two modifications to this graph:
    \begin{enumerate}
        \item \emph{short-cut $(L,E_G)$-incidence graph} is obtained from the $(L, E_G)$-incidence graph by short-cutting the terminals (nodes in $E_G$), where short-cutting a node $e\in E_G$ means adding edges between the neighbours of $e$ so they form a clique.
        
        \item \emph{reduced $(L,E_G)$-incidence graph} is obtained from the short-cut $(L,E_G)$-incidence graph by deleting the set $E_T \setminus T$, where $T$ are the leaf-edges of $E_G$. Here $T$ are the terminals and $L$ are the Steiner nodes.
    \end{enumerate}
\end{definition}

For $J = G \cup L$, we define $\kappa_J(s,t)$ as the maximum number of internally node disjoint $st$-paths in $J$. Given a tree $G = (V,E_G)$, and a set of links $L \subseteq V\times V$, we the $(L,E_G)$-incidence graph $H$, and we call the reduced $(L,E_G)$-incidence graph $H_R$. For distinct vertices $s,t\in V$ we say $(s,t)$ are \emph{$H$-reachable} if $H$ has an $e_se_t$-path (allowing $e_s = e_t$), where $e_s$ and $e_t$ are the corresponding leaf edges of the unique $st$-path in $G$.


\begin{lemma}[\cite{nutov20202nodeconnectivity}]
\label{lemma:connected-block}
    Let $G = (V,E_G)$ be a tree, $L \subseteq V\times V$ be a set of links, and $J = G \cup L$. Let $H$ be the $(L,E_G)$-incidence graph. Then for $s,t\in V$, $\kappa_J (s,t) \geq 2$ if and only if $(s,t)$ are $H$-reachable. Furthermore, $J$ is  $2$-connected if and only if $H_R$ has a path between every two terminals.
\end{lemma}
\begin{proof}
    %here we write down basically the same thing as in nutovs paper. but in my own words and clearer than what he did.
    
    We prove the first statement of the lemma, and let $P$ be the $st$-path in $G$. This statement is proven by induction on the length of $P$, where the length $|P|$ and refers to the number of edges on the path. The case $|P| = 1$ is trivial since $e_s = e_t$ and $s\neq t$. The case $|P| =2$ is the first non-trivial case, and will serve as our base case.
    
    If $|P|=2$ it has $3$ nodes, let $v$ be the middle node of $P$.  Consider $J\setminus \{v\}$ and its two disconnected components $G_s, G_t \subset G\setminus \{v\}$ that contain $s$ and $t$ respectively. Suppose that $\kappa_J(s,t)\geq 2$, then $J\setminus \{v\}$ has an $st$-path. Consider such a path $Q$ that goes through each of the disconnected components $G_s=G_0,G_1,\dots,G_k,G_t=G_{k+1} \subset G\setminus\{v\}$ exactly once; without loss of generality the components are labelled in the order $Q$ visits them. If we label the edges in $G$ that connect $v$ to $G_i$ as $e_i$, then we can see that there must be a link $\ell_i\in L$ between $G_i$ and $G_{i+1}$. Note that by this naming convention and because $|P|=2$, we have $e_0=e_s$ and $e_{k+1}=e_t$. Thus we have the following $st$-path in $H$, that is, $e_s,\ell_0,e_1,\ell_1,\dots,\ell_k,e_t$, and $(s,t)$ are $H$-reachable.
    
    Now suppose $\kappa_J(s,t)=1$, then $J\setminus \{v\}$ has no $st$-path. Let $J_s$ be the component of $J\setminus\{v\}V$ that contains $s$. Let $L_s$ and $L_t$ be the set of links that have both endpoints in $J_s\cup\{v\}$ and $V\setminus J_s$ respectively. Since there is no $st$-path in $J\setminus \{v\}$ it is clear that $L_s$ and $L_t$ partition $L$. In particular, this means for any link $\ell\in L_s$, the path $G_\ell$ shares no edges with any link in $L_t$.    Thus in $H$ there is no path between $L_s$ and $L_t$, and in particular no $e_se_t$ path, and the claim holds.
    
    We now suppose that $|P| \geq 3$, and to prove the claim holds for this case, we first prove several other facts we will need first. Assume that $uv$ and $vt=e_t$ are the last two edges on the $st$-path $P_{st}$, here we assume $P_{xy}$ denotes the subpath of $P$ with endpoints $x$ and $y$. 
    
    For the first fact; suppose we have $\kappa_J(s,t) \geq 2$, we want to show that $\kappa_J(s,v) \geq 2$. Let $C$ be the cycle in $J$ formed by taking the union of the two $st$-paths in $J$. Obviously, if $v\in C$ we have two internally disjoint $sv$-paths in $J$. If $v\notin C$, then pick $a\in P_{sv}$ such that $P_{av}$ only shares a single node with $C$. We claim that $C\cup P_{av}\cup \{v,t\}$ contains two internally disjoint $sv$-paths. In particular, the shortest path in $C$ from $s$ to $a$ then $P_{av}$, then finally the edge $\{v,t\}$, the other path is the remaining $st$-path in $C$.
    
    For the second fact; if $(s,v)$ and $(u,t)$ are both $H$-reachable pairs, we want to show $(s,t)$ are $H$-reachable. To see this, note that there is an $e_se_v$-path and an $e_ve_t$-path in $H$, combining these paths gives the result. 
    
    For the third fact; suppose $(s,t)$ are $H$-reachable, we want to show $(s,v)$ are $H$-reachable. Suppose that $Q$ is the $e_se_t$-path in $H$. We assume for contradiction there is no link $\ell\in L$ that is both on $Q$ and adjacent to $\{u,v\}$. Let $L_s$ and $L_t$ denote the set of links in $L$ with both ends in the connected components of $G-\{uv\}$ containing $s$ and $t$, respectively. The only links not accounted by $L_s$ and $L_t$ are those whose path on $G$ between its endpoints include the edge $\{u,v\}$. In particular, this implies that $Q$ only uses links from $L_s$ and $L_t$, but there is no path between $e_s$ and $e_t$ using only edges from $L_s$ and $L_t$, contradicting the existence of the path $Q$.
    
    Resuming the induction, suppose that $\kappa_J(s,t)\geq 2$, then by the first fact above we know that $\kappa_J(s,v)\geq 2$ and $\kappa_J(u,t)\geq 2$, and by induction we know that $(s,v)$ and $(u,t)$ are $H$-reachable, which by the second fact above means that $(s,t)$ are $H$-reachable. 
    
    Suppose then that $(s,t)$ are $H$-reachable, and assume for contradiction that $\kappa_J(s,t) =1$. By the third fact above we know that $(s,v)$ and $(u,t)$ are $H$-reachable, and by induction we know that $\kappa_J(s,v), \kappa_J(u,t)\geq 2$. Since $\kappa_J(s,t)=1$ we know that there is a node $a\in P\setminus\{s,t\}$ such that $s,t$ are in separate connected components of $J\setminus \{a\}$. If $a\in P_{su}$ this contradicts $\kappa_J(s,v)\geq 2$, while $a\in P_{ut}$ contradicts $\kappa_J(s,v)\geq 2$ if $a=u$ and contradicts $\kappa_J(v,t)\geq 2$ if $a=v$. Thus, we see that $\kappa_J(s,t) \geq 2$, proving the first part of the lemma.
    
    
    For the second part of the Lemma, we first need to observe that $J$ is $2$-node-connected if and only if $\kappa_J(s,t)\geq 2$ for every pair of leaves of $G$. By the first part of the lemma we can see that $J$ is $2$-node-connected if and only if for any 2 leafs $s,t\in G$, $(s,t)$ are $H$-reachable. We obtain the reduced $(L,E_G)$-incidence graph $H_R$ by first short-cutting all the nodes of $G$ and then deleting the nodes corresponding to non-leaf edges. Therefore, for nodes $r,r'\in T$  $(r,r')$ are $H_R$ reachable if and only if $H[F\cup T]$ has an $rr'$-path.
    
\end{proof}

For the reduced $(G, E_G)$-incidence graph $H_R$, consider the Node-Steiner-Tree instance $(H_R,T)$ where the terminals $T$ are the set of leaf-edges from $G$. Fix a feasible solution for this instance, which we call $H'_R$, and suppose the Steiner nodes of this instance are $L'\subseteq L$, we can see the cost of this instance is $|L'|$. By the previous Lemma, we know that $J' = G\cup L'$ is 2-node-connected, thus $L'$ is a feasible solution to the Block-TAP instance $(G,L)$ with cost $|L'|$. 

It remains to see that the Node-Steiner-Tree instance $(H_R, T)$ is in fact a CA-Node-Steiner Tree instance, which can be done by verifying the requirements for a CA-Node-Steiner Tree hold. By definition of the $(L,E_G)$-incidence graph it is clear that terminals are only adjacent to Steiner Nodes. By definition of the short-cut $(L,E_G)$-incidence graph we know that the neighbours of a terminal form a clique. Finally, for link $\ell\in L$ we know that it is adjacent only to the nodes whose corresponding edge in $E_G$ is on that path $T_\ell$, and for any such path, at most two edges are leaf-edges which are all that remain in the reduced $(L,E_G)$-incidence graph. With this, we can conclude Theorem~\ref{cor:approx-preserve-block}.


==> reduction.tex <==
%%%%%%%%%%%%%%%%% REDUCTION TO NODE STEINER TREE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Reducing TAP to Node Steiner Tree instances with certain properties}
Let $T = (V, E)$ be a TAP instance, where $L \subseteq \binom{V}{2}$ is the set of links. Throughout this section, we use the notation $P(\ell) \subseteq E$ to denote the unique path in $T$ connecting the two endpoints of a link $\ell \in L$.  We use the reduction of~\cite{DBLP:conf/stoc/Byrka0A20} in order to reduce the problem to a Node Steiner Tree instance. As a reminder, in the Node Steiner Tree problem, we are given a graph $G$ and a subset of vertices, the terminals, and the goal is to compute a connected subgraph of $G$ that contains all the terminals and minimizes the number of non-terminal vertices contained in it. Such a subgraph can always be assumed to be a tree. We will refer to the number of non-terminal vertices that such a tree contains as the size or cost of the solution.

The way we reduce TAP to Node Steiner Tree is the following. Let $C \subseteq V$ be the set of leaves of $T$. We define the graph $G = (C \cup L, F)$, where we set $C$ to be the set of terminals. The edge set $F$ is defined as follows.
\begin{itemize}
    \item If $\ell \in L$ is a link in $T$ that has a leaf $c \in C$ as an endpoint, then $(\ell, c) \in F$.
    \item Let $\ell_1, \ell_2 \in L$, $\ell_1 \neq \ell_2$. If $P(\ell_1)$ and $P(\ell_2)$ share a vertex, then $(\ell_1, \ell_2) \in F$.
\end{itemize}

We use the notation $N_G(u)$ to denote the set of vertices that are adjacent to a vertex $u$ in $G$. We now describe several properties of the resulting instances, as observed in~\cite{DBLP:conf/stoc/Byrka0A20}.

\begin{observation}[\cite{DBLP:conf/stoc/Byrka0A20}]\label{obs:properties}
\hfill
\begin{enumerate}
    \item For each terminal $c \in C$, we have $N_G(c) \cap C = \emptyset$.
    \item For each Steiner node $\ell \in L$, we have $|N_G(\ell) \cap C| \leq 2$.
    \item For each terminal $c \in C$, the set $N_G(c)$ is a clique in $G$.
    \item If $L' \subseteq L$ is such that $G[C \cup L']$ is connected, then there exists a Steiner Tree in $G[C \cup L']$ connecting the terminals where every terminal is a leaf.
\end{enumerate}
\end{observation}

For completeness, we now prove the following theorem.
\begin{theorem}
Let $T = (V, E)$ be a TAP instance with a set of links $L$, and let $C \subseteq V$ be the set of leaves of $T$. Let $G = (C \cup L, F)$ be the corresponding Node Steiner Tree instance, obtained as described above. Then, there exists a solution of size $k$ for the given TAP instance if and only if there exists a solution of size $k$ for the corresponding Node Steiner Tree instance .
\end{theorem}
\begin{proof}
Let $L' \subseteq L$ be a solution for the TAP instance of size $|L'|$. We will show that $G[C \cup L']$ is a connected graph; if that is the case, then clearly there will be a Steiner tree contained in $G[C \cup L']$ of size at most $|L'|$. For that, consider any pair $c, c' \in C$ of terminals, $c \neq c'$. Let $P(c,c')$ be the unique path connecting $c$ and $c'$ in $T$. Since $L'$ is a feasible solution, every edge $e \in P(s,s')$ is covered by at least one link $\ell \in L'$, meaning that $e \in P(\ell)$. More precisely, let $P(c,c') = (u_0, u_1, \ldots, u_t)$, where $u_0 = c$ and $u_t = c'$. Since $L'$ is a feasible solution, every edge $(u_i, u_{i+1})$, $i = 0, \ldots, t-1$, is covered by a link $\ell_i \in L'$, i.e., $(u_i, u_{i+1}) \in P(\ell_i)$ (we can have $\ell_i = \ell_{i+1}$). This implies that there is an edge between $\ell_i$ and $\ell_{i+1}$ in $G$, for every $i = 0, \ldots, t-1$. Moreover, $\ell_0$ must have $c$ as one of its endpoints, since $c$ is a leaf in $T$, and, similarly, $\ell_{t-1}$ must have $c'$ as one of its endpoints, since $c'$ is a leaf of $T$. Thus, $G[\{c, c'\} \cup \{\ell_0, \ell_1, \ldots, \ell_{t-1}\}]$ will contain a path from $c$ to $c'$. We conclude that there is a Steiner tree connecting all terminals in $G[C \cup L']$, whose size is at most $|L'|$.

Conversely, let $L' \subseteq L$ be a subset of Steiner nodes such that $G[C \cup L']$ contains a Steiner tree connecting the terminals $C$ of cost $|L'|$. We will show that the set of links $L'$ is a feasible solution for the given TAP instance. Suppose otherwise, and let $(u,v) \in E$ be an edge in $T$ that is not covered by any link in $L'$, i.e., $(u,v) \notin P(\ell)$ for every $\ell \in L'$. We now remove the edge $(u,v)$ from $T$, which splits the tree $T$ into two trees $T_u$ and $T_v$. If $T_u = \{u\}$ (i.e., if $u$ is a leaf in $T$), then since $(u,v)$ is not covered, this means that no neighbor of $u$ is included in $L'$, and so $u$ is not connected with the rest of the terminals in $G[C \cup L']$, which is a contradiction. The case where $v$ is a leaf is analyzed in the same way. So, from now on we assume that neither $u$ nor $v$ are leaves in $T$.

Let $c \in T_u \setminus \{u\}$ be a leaf of $T_u$ (in case $u$ is a leaf in $T_u$, then we pick some other leaf) and $c' \in T_v \setminus \{v\}$ be a leaf of $T_v$ (in case $v$ is a leaf in $T_v$, then we pick some other leaf). We will show that there cannot be a path between $c$ and $c'$ in $G[C \cup L']$, which leads to a contradiction. For that, we observe that since $(u,v)$ is not covered by $L'$, it means that the endpoints of every link of $L'$ are contained either both in $T_u$ or both in $T_v$. Let $L_u' \subseteq L'$ be the links whose endpoints are both in $T_u$, and $L_v' \subseteq L'$ be the links whose endpoints are both in $T_v$. We have $L' = L_u' \cup L_v'$. Let $\ell_1 \in L_u'$ and $\ell_2 \in L_v'$. It is clear that $P(\ell_1)$ and $P(\ell_2)$ are vertex disjoint, and so there is no edge connecting a link $\ell_1 \in L_u'$ with a link $\ell_2 \in L_v'$ in $G$. Thus, $G[C \cup L']$ does not connect all terminals, which is a contradiction. We conclude that $L'$ is a feasible set of links for $T$, whose size is $|L'|$.
\end{proof}

It is easy to see that the above theorem is constructive; more precisely, given a Node Steiner Tree solution of size $k$, a TAP solution of size at most $k$ can be found in polynomial time. 

\begin{corollary}\label{cor:approx-preserve}
Let $T = (V, E)$ be a TAP instance with a set of links $L$, and let $C \subseteq V$ be the set of leaves of $T$. Let $G = (C \cup L, F)$ be the corresponding Node Steiner Tree instance, obtained as described above. Then, given an $\alpha$-approximate solution for the Node Steiner Tree instance, one can compute an $\alpha$-approximate solution for the original TAP instance in polynomial time.
\end{corollary}

\begin{observation}
The reduction described above and Corollary~\ref{cor:approx-preserve} hold even if the TAP instance is weighted. In such a case, we end up with a Node Weighted Steiner Tree instance whose weight function describes the weights of the links of the original TAP instance.
\end{observation}


Thus, from now on, we will work with the Node Steiner Tree instances that arise from TAP instances by applying the reduction described above. We will refer to such instances as \textbf{TAP-Node-Steiner-Tree} instances.

Inspired by the techniques that have been applied to the (Edge) Steiner Tree problem (see~\cite{DBLP:journals/siamcomp/BorchersD97}), we will show in the next section that we can decompose an optimal solution of a TAP-Node-Steiner-Tree instance in terms of $k$-restricted components, i.e., components connecting at most $k$ terminals, without losing much in the objective value.


==> resolved_cases.tex <==
\section{Resolved Cases}

In this section we study several special cases. We will often use the fact that the harmonic sum $H(n) \coloneqq \sum_{i = 1}^n \frac{1}{i}$ behaves like a concave function, which is formally shown in the following lemma; its proof is given in Appendix~\ref{appendix:proofs}.
\begin{lemma}[Concavity]\label{lemma:concavity}
Let $n \in \mathbb{N}_{>0}$, $x_i \in \mathbb{N}_{>0}$ and $\lambda_i \in [0,1]$ for $i \in [n]$ such that $\sum_{i = 1}^n \lambda_i = 1$. Then, we have
\begin{equation*}
    \sum_{i = 1}^n \lambda_i H(x_i) \leq H\left(\left\lceil \sum_{i = 1}^n\lambda_i x_i \right\rceil\right).
\end{equation*}
\end{lemma}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{H-average of a Star is bounded by $H(2) + o(1)$}

We define a particular instance of the TAP-Node-Steiner-Tree problem that we call a ``star". Let $t \geq 2$ be an integer parameter, and assume we have $2t$ many terminals $\{r_i^{(1)}, r_i^{(2)}\}_{i = 1}^t$, and $t$ Steiner nodes $\{s_1, \ldots, s_t\}$, where $s_i$ is adjacent to terminals $r_i^{(1)}, r_i^{(2)}$ for every $i \in [t]$. There is also an additional Steiner node $s_0$ that is adjacent to every other Steiner node $s_1, \ldots, s_t$, but adjacent to no terminals. 

We will show that there is a terminal spanning tree that gives an average $H$-average of at most $H(2)$. Consider the following terminal spanning tree:
\begin{itemize}
    \item There is an edge between $r_i^{(1)}$ and $r_i^{(2)}$ for every $i \in [t]$.
    \item For every $i = 2, \ldots, t$, there is an edge between $r_i^{(1)}$ and $r_1^{(1)}$.
\end{itemize}

It is easy to see that the w-value of the root $s_0$ is $t-1$, the $w$-value of $r_1$ is $t$, and every other Steiner node has $w$-value $2$. Thus, the $w$-average is
\[
    \frac{1}{t+1} \sum_{i = 0}^t w(s_i) = \frac{(t-1)+t+(t-1)2}{t+1} = \frac{4t-3}{t+1} = 4 - \frac{7}{t+1} \rightarrow 4.
\]

By concavity (see Lemma~\ref{lemma:concavity}), this immediately implies that the $H$-average is at most $H(4)$. But this is not good enough, so we instead look directly at the $H$-average
\[
    \frac{1}{t+1} \sum_{i = 0}^t H(w(s_i)) = \frac{H(t-1)+H(t)+(t-1)H(2)}{t+1} = H(2) + \frac{H(t-1)+H(t) - 2H(2)}{t+1} \rightarrow H(2).
\]
Moreover, it is easy to see that the $H$-average is at most $H(3)$, even for small values of $t \geq 2$. This is because we always have
\begin{equation*}
    \frac{H(t-1)+ H(t) - 2H(2)}{t+1} \leq \frac{1}{3}.
\end{equation*}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Binary Tree bounded by $1.77$}
To show that the $H$-average of any binary tree is at most the stated bound we will make use of the following lemma.
\begin{lemma}
Given a binary tree with $n$ vertices, where only the leaves may be final nodes, the number of vertices with $w$-value $w\in \{2, 3, \dots, i\}$ is at least 
\[
    \lceil (n+1)(1 - \frac{1}{2^{i-1}} \rceil
\]
where $i$ is at most $\lceil \log_2 (n+1) \rceil$
\end{lemma}
\begin{proof}

\end{proof}
Given this lemma, we can show the claimed bound easily by showing that the total $H$-average is at most 
\[
    \sum^{\lceil \log_2 (n+1) \rceil}_{i=1}\frac{n+1}{2^i}H(i+1) \leq (n+1)\sum^\infty_{i=1}\frac{H(i+1)}{2^i} < 1.77(n+1)
\]



%The idea here ought to be by concavity. It is. 

For this section we assume that we have a rooted Complete Binary Tree $G$ with $q+2$ levels, $0, 1, 2,\dots, q, q+1$. We assume that there are $2^{q+1} = 2t$ many terminals $\{r_i^{(1)}, r_i^{(2)}\}^t_{i=1}$, and each pair of terminals  $\{r_i^{(1)}, r_i^{(2)}\}$ is adjacent to a node $s_i$ on the $q+1$ level. We will find a terminal spanning tree by marking edges in the following way: from every node, mark the edge to its left child. To find the terminal spanning tree with these marked edges, for every terminal to terminal path in $G$ with exactly one unmarked edge, we add an edge to the terminal spanning tree. 

By summing across each row one by one it's not hard to show that the average of the $H$-values in this tree is the following
\[
    \frac{1}{2^{q+1}-1}\left( 1 + \sum_{l=1}^{q} \left[ H(l + 1) + \sum_{i=1}^{l} 2^{l-i} H(i+1) \right] \right) 
\]
\[
    = \frac{1}{2^{q+ 1}- 1}\left( 1 + \left[ 2H(q+1) + 2^2H(q) + \dots + 2^qH(2) + H(1)   \right]\right)
\]  
\[
    = \frac{1}{2^{q+ 1}- 1}\left(1 + \left[ \sum^q_{l=1}2^{q-l+1}H(i+1)  \right]\right)
    = \frac{1}{2^{q+ 1}- 1} +  \sum^q_{l=1}\frac{2^{q-l+1}H(i+1)}{2^{q+ 1}- 1 }
\]
\[  
    = \frac{1}{2^{q+ 1}- 1} + \sum^q_{i =1}\frac{H(i+1) }{2^{l}( 1-\frac{1}{2^{q+1}})} \leq  \frac{1}{2^{q+ 1}- 1} + 1.02259
\]  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Every Steiner Node is Adjacent to a Terminal}
In this section, we consider TAP-Node-Steiner-Tree instances where each Steiner Node is adjacent to at least one terminal. More precisely, we consider instances with $t = t_1 + t_2$ Steiner nodes $s_1, \ldots, s_t$, and $2t - t_1$ terminals, where for $i = 1, \ldots, t_1$, each $s_i$ is adjacent to exactly one terminal $r_i^{(1)}$, and for each $i = t_1 + 1, \ldots, t$, each $s_i$ is adjacent to two terminals  $\{r_i^{(1)},r_i^{(2)}\}^t_{i= t_1 + 1}$. The subgraph of Steiner nodes may be any tree with $t$ vertices. For such Steiner trees, we define the \textbf{tree-following terminal spanning tree} as follows:
\begin{itemize}
    \item There is an edge between $r_i^{(1)}$ and $r_i^{(2)}$ for every $i=t_1 + 1,\dots, t$.
    \item For two adjacent Steiner nodes $s_i$ and $s_j$, there is an edge between $r_i^{(1)}$ and $r_j^{(1)}$.
\end{itemize}

We will prove the following theorem.
\begin{theorem}\label{thm:every-steiner-is-final-upper-bound}
Let $T$ be a TAP-Node-Steiner-Tree instance where every Steiner node is adjacent to at least one terminal. Then, the tree-following terminal spanning tree has $w$ values that satisfy
\begin{equation*}
\frac{1}{|S|} \sum_{s \in S} H(w(s)) \leq H(3).
\end{equation*}
\end{theorem}
\begin{proof}
Consider the tree-following terminal spanning tree. It is easy to see that every Steiner node $s$ has $w$-value $d(s)-1$, where $d(s)$ denotes the degree of the node (in the original tree). Thus, we have
\begin{align*}
    \frac{1}{t} \sum_{i = 1}^t w(s_i) &= \frac{1}{t} \left( \sum_{i = 1}^t d(s) - t \right) = \frac{2(t + 2t - t_1 - 1) - (2t - t_1)}{t} - 1\\
    &= \frac{4t - t_1 - 2}{t} - 1 = 3 - \frac{t_1 + 2}{t} < 3.
\end{align*}
Finally, by concavity (Lemma~\ref{lemma:concavity}), we get that
\begin{equation*}
    \frac{1}{t} \sum_{i = 1}^t H(w(s_i)) \leq H\left( \left \lceil \frac{1}{t} \sum_{i = 1}^t w(s_i)    \right\rceil  \right) = H(3).
\end{equation*}
\end{proof}

We will now show that the tree-following terminal spanning tree is indeed optimal with respect to minimizing $\frac{1}{|S|} \sum_{s \in S} H(w(s))$.
\begin{lemma}\label{lemma:tree-following-optimal}
Let $T$ be a TAP-Node-Steiner-Tree instance where every Steiner node is adjacent to at least one terminal. Then, the tree-following terminal spanning tree $\mathcal{O}$ is the optimal terminal spanning tree with respect to minimizing $\frac{1}{|S|} \sum_{s \in S} H(w(s))$.
\end{lemma}
\begin{proof}
The goal will be to show that replacing an edge of a terminal spanning tree that is not tree-following with one that is will always reduce the sum of $w$ values. 

Consider a terminal spanning tree $Y$ that is not tree-following. Since $Y$ is not tree-following there is an edge $e = \{r_i^{(1)}, r_j^{(1)}\}$ such that the path $r_i^{(1)} \rightarrow r_j^{(1)}$ in $T$ passes Steiner node $s_k$ with adjacent an adjacent terminal. Removing $e$ from $Y$ we get disjoint components $Y_1$ and $Y_2$, and we assume without loss of generality that $r_i^{(1)}\in Y_1$ and $r_k^{(1)}, r_j^{(1)} \in Y_2$. 

Adding edge $e' = \{r_i^{(1)}, r_k^{(1)}\}$ to $Y_1\cup Y_2$ we get a new terminal spanning tree $Y' = Y_1\cup Y_2\cup \{e'\}$.  The edge $e$ causes $w(v)$ to increase by one for every Steiner node $v$ on the path  $ s_i \rightarrow s_j$ in $T$. The edge $e'$ causes the $w(v)$ values to increase by one for every Steiner node $v$ on the path $s_k \rightarrow s_i$ instead. Thus the sum of the $w$ terms is decreased. 
\end{proof}


Finally, we show that the $H(3)$ bound that we showed in Theorem~\ref{thm:every-steiner-is-final-upper-bound} is tight. More formally, we prove the following.
\begin{lemma}\label{lemma:bad-example-H(3)}
For any $\varepsilon > 0$, there exist TAP-Node-Steiner-Tree instances where every Steiner node is adjacent to at least one terminal, such that the corresponding tree-following terminal spanning tree has average $H(w)$ value strictly larger than $H(3) - \varepsilon$.
\end{lemma}
\begin{proof}
Consider the following graph. Let $t = \lceil \frac{2}{3\varepsilon} \rceil + 1$ and let $s_1, \ldots, s_t$ be the set of Steiner nodes. For every $i = 2, \ldots, t-1$, the node $s_i$ is adjacent to $s_{i-1}$ and $s_{i+1}$. In other words, the nodes $s_1, \ldots, s_t$ form a path whose endpoints are $s_1$ and $s_t$. Finally, every Steiner node $s_i$ is adjacent to two terminals $r_i^{(1)}$ and $r_i^{(2)}$. It is easy to see that the tree-following terminal spanning tree results in the following $w$-values:
\begin{itemize}
    \item $w(s_1) = w(s_t) = 2$.
    \item $w(s_i) = 3$ for every $i = 2, \ldots, t-1$.
\end{itemize}
Thus,
\begin{equation*}
\frac{1}{t} \sum_{i = 1}^t H(w(s_i)) =  \frac{2H(2) + (t-2) H(3)}{t} = H(3) - \frac{2}{3t} > H(3) - \varepsilon.
\end{equation*}
\end{proof}

Thus, Lemmas~\ref{lemma:tree-following-optimal} and \ref{lemma:bad-example-H(3)} imply the following.
\begin{observation}
By using our current techniques, the best we can hope for is $H(3)$.
\end{observation}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Any TAP-Node-Steiner-Tree is bounded by $H(4)$}
In this section we will show that any TAP-Node-Steiner-Tree instance is bounded by $H(4)$. We assume that we have $s+t$ Steiner Nodes, and that $t = t_1 + t_2$ Steiner nodes are those nodes that are adjacent to terminals, and that there are $2t - t_1$ many terminals. These Steiner nodes that are adjacent to terminals we denote by $\mathcal{F}$. We enumerate the nodes of $\mathcal{F}$ the following way: for $i = 1, \ldots, t_1$, each $s_i$ is adjacent to exactly one terminal $r_i^{(1)}$, and for each $i = t_1 + 1, \ldots, t$, each $s_i$ is adjacent to two terminals  $\{r_i^{(1)},r_i^{(2)}\}$. The remaining Steiner nodes are enumerated $\{s_i \}_{i=t+1}^{t+s}$. 
We will first show this claim for instances where the only nodes of $\mathcal{F}$ are leaves, then extend the argument to include interior nodes in $\mathcal{F}$.

Our approach will be to use an Eulerian tour of the subgraph induced by the Steiner nodes to find the edges of the terminal spanning tree. To do this, we will consider the subtree $S$ formed by the Steiner nodes. note that obviously $S$ is a connected subtree since we assume that terminals are leaves of $G$. Next we create a duplicate edge $e'$ for every edge $e \in E(S)$, calling this new graph $S'$. We then use an Eulerian Tour $\mathcal{T}$ of $S'$ to find the edges of the terminal spanning tree in the following way: 

\begin{itemize}
    \item $w$-value of every node is initially $0$
    \item Starting from a node $s_i \in \mathcal{F}$ we follow $\mathcal{T}$ until the next node $s_j \in \mathcal{F}$
    \item Add edge $\{ r_i^{(1)}, r_j^{(1)} \}$ to the terminal spanning tree
    \item Repeat the previous two steps until each node of $\mathcal{F}$ has been reached
    \item For every node $\{s_i\}_{i=t_1+1}^{t}$, we add edge $\{r_i^{(1)}, r_i^{(2)}\}$ to the terminal spanning tree
\end{itemize}

The $w$-value of a node $s$ that is not in $\mathcal{F}$ is the number of times the tour $\mathcal{T}$ passes it, which is $d(s)$, the degree of $s$. The nodes in $\mathcal{F}$ have a $w$-value equal to their degree in $S'$ since there is a terminal spanning tree edge corresponding to every adjacent edge of $s$ in $S'$. For every node $\{s_i\}_{i=t_1+1}^{t}$ the $w$-value is increased by $1$. If we let $d_S(v)$ denote the degree of $v$ in $S$ then the average $w$-value of the nodes in $S$ is
      
\begin{align*}
                \frac{1}{|S|}\left( \sum_{i=1}^{t_1}(d_S(s_i) + 1) + \sum_{i=t_1 + 1}^t (d_S(s_i) + 2) + \sum_{i = t+1}^{s+t}d_S(s_i)  \right) &=  \frac{1}{|S|}\left( t_1 + 2t_2 + \sum_{i=1}^{s+t}d_S(s_i) \right) \\
                &= \frac{1}{|S|}\left( t_1 + 2t_2 + 2(|S| - 1) \right) \\
                &= 2 + \frac{t_1 + 2t_2 -2}{s + t_1 + t_2} \\
                &\leq 2 + 2\frac{s + t_1 + t_2 - 1}{s + t_1 + t_2} \\
                &= 4 - \frac{2}{|S|}\\
\end{align*}

%%%%
% the formula above but in two lines
%%%%
%\[
%    \frac{1}{|S|}\left( \sum_{i=1}^{t_1}(d_S(s_i) + 1) + \sum_{i=t_1 + 1}^t (d_S(s_i) + 2) + \sum_{i = t+1}^{s+t}d_S(s_i)  \right) =  \frac{1}{|S|}\left( t_1 + 2t_2 + \sum_{i=1}^{s+t}d_S(s_i) \right)
%\]
%\[
%    = \frac{1}{|S|}\left( t_1 + 2t_2 + 2(|S| - 1) \right) = 2 + \frac{t_1 + 2t_2 -2}{s + t_1 + t_2} \leq 2 + 2\frac{s + t_1 + t_2 - 1}{s + t_1 + t_2} = 4 - \frac{2}{|S|}
%\]

Now it remains to modify the procedure to allow for interior nodes that are adjacent to terminals. The issue with the original procedure is that we create an edge every time the tour $\mathcal{T}$ enters and leaves a node $s$ that is adjacent to a terminal. This is fine when $\mathcal{F}$ is only leaves, but can be an issue if $\mathcal{F}$ contains interior nodes with higher degree. The solution for this issue is simple; only create an edge when $\mathcal{T}$ arrives at an interior node in $\mathcal{T}$, but do not create when it leaves. We let $t_1 = t_1^{in} + t_1^l$ and $t_2 = t_2^{in} + t_2^l$, where $\{s_i\}_{i=1}^{t_1^{in}}$ and $\{s_i\}_{i=t_1 + 1}^{t_1+t_2^{in}}$ are the interior nodes, and $\{s_i\}_{i= t_1^{in} +1}^{t_1}$ and $\{s_i\}_{i= t_1+t_2^{in}}^{t}$ are the leaves.
\[
    \frac{1}{|S|}\left( \sum_{i=1}^{t_1^{in}}(d_S(s_i)) + \sum_{i= t_1^{in} + 1}^{t_1} (d_S(s_i) + 1) +\sum_{i = t_1 +1}^{t_1 + t_2^{in}} (d_S(s_i)+1) + \sum_{i = t_1 + t_2^{in} +1}^{t}(d_S(s_i) + 2) + \sum_{i= t+1}^{s+t}d_S(s_i) \right) 
\]
\[
    = \frac{1}{|S|}\left( \sum_{s \in S}d_S(s) + t_1^l + t_2 + 2t_2^l \right) = \frac{1}{|S|}\left( 2|S| - 2 + t^l_1 + t_2 + 2t^l_2  \right)
\]
\[
    = 2 + \frac{t_1^l + t_2 + 2t^l_2}{s + t_1 + t_1^l + t_2 + t_2^l} - \frac{2}{|S|} \leq 4 - \frac{2}{|S|}
\]


Notice that if $s \geq t_2$ then the above is in fact bounded by $3$, just as when $s = 0$. 

